Language Model Probabilities are Not Calibrated in Numeric Contexts

Some statements have one well-defined continuation (e.g., "the Eiffel Tower is in [Paris]"), whereas others have a natural distribution over multiple options (e.g., "the weighted coin flip was [Heads/Tails].") We argue that language model (LM) outputs should capture these natural distributions. Our work specifically tests whether LM output probabilities are calibrated to numeric information within their textual contexts. For example, if the context (the prompt) concerns two equally likely options (e.g., heads or tails for a fair coin), the LM output probabilities should also be equal. Likewise, in a context with nonuniformly likely events (e.g., rolling a pair with two dice) an LM should output proportionate probabilities. However, we find that even in simple settings, the best LMs (1) are poorly calibrated and (2) have systematic biases: artifacts like word identity, word order, and word frequency all impact calibration. For example, gpt-4o-mini often picks the first of two options presented in the prompt regardless of the options' implied likelihoods, whereas Llama-3.1-8B picks the second. Models do not allocate probability mass among valid options in a calibrated manner.

==> archive/arr_color_rankings.tex <==
\begin{table*}[ht!]
\scriptsize
\centering

\begin{tabular}{@{}l@{\hspace{2pt}}l@{\hspace{3.75pt}}l@{\hspace{3.75pt}}@{\hspace{3.75pt}}l@{\hspace{3.75pt}}l@{\hspace{3.75pt}}l@{\hspace{3.75pt}}l@{\hspace{3.75pt}}l@{\hspace{3.75pt}}l@{\hspace{3.75pt}}l@{\hspace{3.75pt}}l@{\hspace{3.75pt}}l@{}}
\toprule
& \multicolumn{2}{@{}l}{\textit{Color Rank}} \\
 &                                                    R0&    R1  &                                                        R2  &                                                        R3  &                                                        R4  &                                                       R5  &                                                       R6  &                                                        R7  &                                                        R8  &                                                        R9  &                                                         R10 \\
\midrule
Mistral-7B-v0.3   &   \textcolor{gray}{\rule{0.15cm}{0.15cm}} &    \textcolor{green}{\rule{0.15cm}{0.15cm}}  0/1  {\tiny (+0.03)} &      \textcolor{red}{\rule{0.15cm}{0.15cm}}  1/2 {\tiny (+0.01)} &  \textcolor{orange}{\rule{0.15cm}{0.15cm}}  2/3 {\tiny (-0.04)} &    \textcolor{pink}{\rule{0.15cm}{0.15cm}}  3/4 {\tiny (-0.04)} &  \textcolor{purple}{\rule{0.15cm}{0.15cm}}  2/5 {\tiny (-0.00)} &   \textcolor{black}{\rule{0.15cm}{0.15cm}}  4/6 {\tiny (-0.04)} &     \textcolor{gold}{\rule{0.15cm}{0.15cm}}  1/7 {\tiny (+0.01)} &  \textcolor{yellow}{\rule{0.15cm}{0.15cm}}  5/8 {\tiny (-0.02)} &     \textcolor{blue}{\rule{0.15cm}{0.15cm}}  2/9 {\tiny (+0.01)} &   \textcolor{brown}{\rule{0.15cm}{0.15cm}}  5/10 {\tiny (-0.01)} \\
gpt-4-turbo       &   \textcolor{gray}{\rule{0.15cm}{0.15cm}} &   \textcolor{brown}{\rule{0.15cm}{0.15cm}}  0/1 {\tiny (-0.01)} &    \textcolor{pink}{\rule{0.15cm}{0.15cm}}  2/2 {\tiny (-0.07)} &    \textcolor{gold}{\rule{0.15cm}{0.15cm}}  3/3 {\tiny (-0.06)} &   \textcolor{green}{\rule{0.15cm}{0.15cm}}  4/4 {\tiny (-0.09)} &  \textcolor{purple}{\rule{0.15cm}{0.15cm}}  4/5 {\tiny (-0.05)} &     \textcolor{red}{\rule{0.15cm}{0.15cm}}  5/6 {\tiny (-0.04)} &   \textcolor{black}{\rule{0.15cm}{0.15cm}}  5/7 {\tiny (-0.01)} &  \textcolor{orange}{\rule{0.15cm}{0.15cm}}  5/8 {\tiny (-0.05)} &    \textcolor{blue}{\rule{0.15cm}{0.15cm}}  6/9 {\tiny (-0.04)} &  \textcolor{yellow}{\rule{0.15cm}{0.15cm}}  7/10 {\tiny (-0.03)} \\
\midrule
Meta-Llama-3.1-8B &   \textcolor{black}{\rule{0.15cm}{0.15cm}} &  \textcolor{orange}{\rule{0.15cm}{0.15cm}}  1/1 {\tiny (-0.04)} &  \textcolor{yellow}{\rule{0.15cm}{0.15cm}}  2/2 {\tiny (-0.04)} &     \textcolor{blue}{\rule{0.15cm}{0.15cm}}  0/3 {\tiny (+0.02)} &   \textcolor{gray}{\rule{0.15cm}{0.15cm}}  4/4 {\tiny (-0.06)} &    \textcolor{gold}{\rule{0.15cm}{0.15cm}}  3/5 {\tiny (-0.05)} &   \textcolor{green}{\rule{0.15cm}{0.15cm}}  4/6 {\tiny (-0.03)} &   \textcolor{brown}{\rule{0.15cm}{0.15cm}}  2/7 {\tiny (-0.02)} &  \textcolor{purple}{\rule{0.15cm}{0.15cm}}  6/8 {\tiny (-0.03)} &    \textcolor{pink}{\rule{0.15cm}{0.15cm}}  7/9 {\tiny (-0.05)} &     \textcolor{red}{\rule{0.15cm}{0.15cm}}  7/10 {\tiny (-0.05)} \\
Mistral-7B-v0.1   &  \textcolor{orange}{\rule{0.15cm}{0.15cm}} &    \textcolor{pink}{\rule{0.15cm}{0.15cm}}  1/1 {\tiny (-0.02)} &   \textcolor{purple}{\rule{0.15cm}{0.15cm}}  0/2 {\tiny (+0.07)} &   \textcolor{gray}{\rule{0.15cm}{0.15cm}}  3/3 {\tiny (-0.11)} &      \textcolor{red}{\rule{0.15cm}{0.15cm}}  1/4 {\tiny (+0.05)} &  \textcolor{yellow}{\rule{0.15cm}{0.15cm}}  3/5 {\tiny (-0.00)} &    \textcolor{green}{\rule{0.15cm}{0.15cm}}  2/6 {\tiny (+0.02)} &    \textcolor{brown}{\rule{0.15cm}{0.15cm}}  3/7 {\tiny (+0.00)} &    \textcolor{gold}{\rule{0.15cm}{0.15cm}}  7/8 {\tiny (-0.06)} &     \textcolor{blue}{\rule{0.15cm}{0.15cm}}  3/9 {\tiny (+0.03)} &   \textcolor{black}{\rule{0.15cm}{0.15cm}}  5/10 {\tiny (-0.01)} \\
Mixtral-8x7B-v0.1 &    \textcolor{blue}{\rule{0.15cm}{0.15cm}} &   \textcolor{green}{\rule{0.15cm}{0.15cm}}  1/1 {\tiny (-0.10)} &  \textcolor{purple}{\rule{0.15cm}{0.15cm}}  1/2 {\tiny (-0.02)} &     \textcolor{red}{\rule{0.15cm}{0.15cm}}  3/3 {\tiny (-0.04)} &    \textcolor{gold}{\rule{0.15cm}{0.15cm}}  3/4 {\tiny (-0.08)} &   \textcolor{black}{\rule{0.15cm}{0.15cm}}  2/5 {\tiny (-0.03)} &   \textcolor{gray}{\rule{0.15cm}{0.15cm}}  5/6 {\tiny (-0.04)} &  \textcolor{yellow}{\rule{0.15cm}{0.15cm}}  3/7 {\tiny (-0.02)} &   \textcolor{brown}{\rule{0.15cm}{0.15cm}}  6/8 {\tiny (-0.06)} &  \textcolor{orange}{\rule{0.15cm}{0.15cm}}  8/9 {\tiny (-0.06)} &   \textcolor{pink}{\rule{0.15cm}{0.15cm}}  10/10 {\tiny (-0.06)} \\
Yi-1.5-34B        &   \textcolor{brown}{\rule{0.15cm}{0.15cm}} &    \textcolor{black}{\rule{0.15cm}{0.15cm}}  0/1 {\tiny (+0.01)} &   \textcolor{orange}{\rule{0.15cm}{0.15cm}}  1/2 {\tiny (+0.00)} &   \textcolor{yellow}{\rule{0.15cm}{0.15cm}}  0/3 {\tiny (+0.02)} &     \textcolor{blue}{\rule{0.15cm}{0.15cm}}  0/4 {\tiny (+0.02)} &     \textcolor{gold}{\rule{0.15cm}{0.15cm}}  0/5 {\tiny (+0.04)} &  \textcolor{purple}{\rule{0.15cm}{0.15cm}}  3/6 {\tiny (-0.01)} &   \textcolor{green}{\rule{0.15cm}{0.15cm}}  5/7 {\tiny (-0.04)} &     \textcolor{red}{\rule{0.15cm}{0.15cm}}  8/8 {\tiny (-0.07)} &    \textcolor{pink}{\rule{0.15cm}{0.15cm}}  5/9 {\tiny (-0.04)} &   \textcolor{gray}{\rule{0.15cm}{0.15cm}}  8/10 {\tiny (-0.07)} \\
Yi-1.5-9B         &  \textcolor{orange}{\rule{0.15cm}{0.15cm}} &  \textcolor{purple}{\rule{0.15cm}{0.15cm}}  0/1 {\tiny (-0.01)} &    \textcolor{blue}{\rule{0.15cm}{0.15cm}}  1/2 {\tiny (-0.01)} &    \textcolor{pink}{\rule{0.15cm}{0.15cm}}  2/3 {\tiny (-0.02)} &  \textcolor{yellow}{\rule{0.15cm}{0.15cm}}  3/4 {\tiny (-0.02)} &     \textcolor{red}{\rule{0.15cm}{0.15cm}}  3/5 {\tiny (-0.04)} &   \textcolor{brown}{\rule{0.15cm}{0.15cm}}  5/6 {\tiny (-0.04)} &    \textcolor{gold}{\rule{0.15cm}{0.15cm}}  2/7 {\tiny (-0.02)} &   \textcolor{gray}{\rule{0.15cm}{0.15cm}}  5/8 {\tiny (-0.04)} &   \textcolor{black}{\rule{0.15cm}{0.15cm}}  6/9 {\tiny (-0.04)} &   \textcolor{green}{\rule{0.15cm}{0.15cm}}  8/10 {\tiny (-0.05)} \\
gemma-2-27b       &   \textcolor{brown}{\rule{0.15cm}{0.15cm}} &  \textcolor{yellow}{\rule{0.15cm}{0.15cm}}  1/1 {\tiny (-0.04)} &    \textcolor{blue}{\rule{0.15cm}{0.15cm}}  1/2 {\tiny (-0.01)} &  \textcolor{orange}{\rule{0.15cm}{0.15cm}}  2/3 {\tiny (-0.02)} &  \textcolor{purple}{\rule{0.15cm}{0.15cm}}  4/4 {\tiny (-0.03)} &   \textcolor{green}{\rule{0.15cm}{0.15cm}}  4/5 {\tiny (-0.03)} &   \textcolor{black}{\rule{0.15cm}{0.15cm}}  5/6 {\tiny (-0.02)} &     \textcolor{red}{\rule{0.15cm}{0.15cm}}  4/7 {\tiny (-0.02)} &   \textcolor{gray}{\rule{0.15cm}{0.15cm}}  6/8 {\tiny (-0.04)} &    \textcolor{pink}{\rule{0.15cm}{0.15cm}}  8/9 {\tiny (-0.04)} &   \textcolor{gold}{\rule{0.15cm}{0.15cm}}  10/10 {\tiny (-0.05)} \\
gemma-2-9b        &    \textcolor{blue}{\rule{0.15cm}{0.15cm}} &  \textcolor{purple}{\rule{0.15cm}{0.15cm}}  1/1 {\tiny (-0.09)} &     \textcolor{red}{\rule{0.15cm}{0.15cm}}  2/2 {\tiny (-0.15)} &    \textcolor{pink}{\rule{0.15cm}{0.15cm}}  3/3 {\tiny (-0.14)} &   \textcolor{green}{\rule{0.15cm}{0.15cm}}  4/4 {\tiny (-0.16)} &   \textcolor{brown}{\rule{0.15cm}{0.15cm}}  4/5 {\tiny (-0.14)} &  \textcolor{orange}{\rule{0.15cm}{0.15cm}}  6/6 {\tiny (-0.13)} &  \textcolor{yellow}{\rule{0.15cm}{0.15cm}}  7/7 {\tiny (-0.16)} &    \textcolor{gold}{\rule{0.15cm}{0.15cm}}  8/8 {\tiny (-0.13)} &   \textcolor{black}{\rule{0.15cm}{0.15cm}}  9/9 {\tiny (-0.19)} &  \textcolor{gray}{\rule{0.15cm}{0.15cm}}  10/10 {\tiny (-0.29)} \\
gpt-3.5           &   \textcolor{green}{\rule{0.15cm}{0.15cm}} &      \textcolor{red}{\rule{0.15cm}{0.15cm}}  0/1 {\tiny (+0.01)} &  \textcolor{yellow}{\rule{0.15cm}{0.15cm}}  1/2 {\tiny (-0.03)} &  \textcolor{orange}{\rule{0.15cm}{0.15cm}}  3/3 {\tiny (-0.03)} &    \textcolor{pink}{\rule{0.15cm}{0.15cm}}  3/4 {\tiny (-0.04)} &    \textcolor{gold}{\rule{0.15cm}{0.15cm}}  4/5 {\tiny (-0.05)} &    \textcolor{blue}{\rule{0.15cm}{0.15cm}}  3/6 {\tiny (-0.01)} &   \textcolor{brown}{\rule{0.15cm}{0.15cm}}  5/7 {\tiny (-0.03)} &   \textcolor{gray}{\rule{0.15cm}{0.15cm}}  6/8 {\tiny (-0.04)} &   \textcolor{black}{\rule{0.15cm}{0.15cm}}  6/9 {\tiny (-0.02)} &  \textcolor{purple}{\rule{0.15cm}{0.15cm}}  8/10 {\tiny (-0.04)} \\
gpt-4o            &    \textcolor{blue}{\rule{0.15cm}{0.15cm}} &     \textcolor{red}{\rule{0.15cm}{0.15cm}}  1/1 {\tiny (-0.05)} &   \textcolor{green}{\rule{0.15cm}{0.15cm}}  2/2 {\tiny (-0.05)} &  \textcolor{yellow}{\rule{0.15cm}{0.15cm}}  2/3 {\tiny (-0.02)} &  \textcolor{purple}{\rule{0.15cm}{0.15cm}}  3/4 {\tiny (-0.04)} &  \textcolor{orange}{\rule{0.15cm}{0.15cm}}  4/5 {\tiny (-0.03)} &    \textcolor{pink}{\rule{0.15cm}{0.15cm}}  6/6 {\tiny (-0.05)} &   \textcolor{black}{\rule{0.15cm}{0.15cm}}  7/7 {\tiny (-0.04)} &   \textcolor{gray}{\rule{0.15cm}{0.15cm}}  7/8 {\tiny (-0.04)} &   \textcolor{brown}{\rule{0.15cm}{0.15cm}}  9/9 {\tiny (-0.06)} &   \textcolor{gold}{\rule{0.15cm}{0.15cm}}  10/10 {\tiny (-0.06)} \\
gpt-4o-mini       &  \textcolor{orange}{\rule{0.15cm}{0.15cm}} &  \textcolor{purple}{\rule{0.15cm}{0.15cm}}  0/1 {\tiny (-0.01)} &    \textcolor{pink}{\rule{0.15cm}{0.15cm}}  2/2 {\tiny (-0.06)} &  \textcolor{yellow}{\rule{0.15cm}{0.15cm}}  3/3 {\tiny (-0.03)} &     \textcolor{red}{\rule{0.15cm}{0.15cm}}  3/4 {\tiny (-0.04)} &    \textcolor{blue}{\rule{0.15cm}{0.15cm}}  5/5 {\tiny (-0.07)} &   \textcolor{green}{\rule{0.15cm}{0.15cm}}  6/6 {\tiny (-0.05)} &    \textcolor{gold}{\rule{0.15cm}{0.15cm}}  7/7 {\tiny (-0.07)} &   \textcolor{black}{\rule{0.15cm}{0.15cm}}  8/8 {\tiny (-0.12)} &   \textcolor{brown}{\rule{0.15cm}{0.15cm}}  9/9 {\tiny (-0.13)} &  \textcolor{gray}{\rule{0.15cm}{0.15cm}}  10/10 {\tiny (-0.14)} \\

% Avg Rank & \textcolor{orange}{\rule{0.15cm}{0.15cm}} orange & \textcolor{blue}{\rule{0.15cm}{0.15cm}} blue & \textcolor{purple}{\rule{0.15cm}{0.15cm}} purple & \textcolor{green}{\rule{0.15cm}{0.15cm}} green & \textcolor{red}{\rule{0.15cm}{0.15cm}} red & \textcolor{yellow}{\rule{0.15cm}{0.15cm}} yellow & \textcolor{pink}{\rule{0.15cm}{0.15cm}} pink & \textcolor{brown}{\rule{0.15cm}{0.15cm}} brown & \textcolor{gray}{\rule{0.15cm}{0.15cm}} white & \textcolor{black}{\rule{0.15cm}{0.15cm}} black & \textcolor{gold}{\rule{0.15cm}{0.15cm}} gold\\
\midrule
\textit{Avg Rank} & \textcolor{orange}{\rule{0.15cm}{0.15cm}}  & \textcolor{blue}{\rule{0.15cm}{0.15cm}} blue & \textcolor{purple}{\rule{0.15cm}{0.15cm}} purple & \textcolor{yellow}{\rule{0.15cm}{0.15cm}} yellow & \textcolor{red}{\rule{0.15cm}{0.15cm}} red & \textcolor{green}{\rule{0.15cm}{0.15cm}} green & \textcolor{pink}{\rule{0.15cm}{0.15cm}} pink & \textcolor{brown}{\rule{0.15cm}{0.15cm}} brown & \textcolor{black}{\rule{0.15cm}{0.15cm}} black & \textcolor{gray}{\rule{0.15cm}{0.15cm}} white & \textcolor{gold}{\rule{0.15cm}{0.15cm}} gold \\

%Meta-Llama-3.1-8B &  \textcolor{orange}{\rule{0.15cm}{0.15cm}} 1/1 {\tiny (-0.04)} &  \textcolor{yellow}{\rule{0.15cm}{0.15cm}}  2/2 {\tiny (-0.04)} &     \textcolor{blue}{\rule{0.15cm}{0.15cm}}  0/3 {\tiny (+0.02)} &   \textcolor{gray}{\rule{0.15cm}{0.15cm}}  4/4 {\tiny (-0.06)} &    \textcolor{gold}{\rule{0.15cm}{0.15cm}}  3/5 {\tiny (-0.05)} &   \textcolor{green}{\rule{0.15cm}{0.15cm}}  4/6 {\tiny (-0.03)} &   \textcolor{brown}{\rule{0.15cm}{0.15cm}}  2/7 {\tiny (-0.02)} &  \textcolor{purple}{\rule{0.15cm}{0.15cm}}  6/8 {\tiny (-0.03)} &    \textcolor{pink}{\rule{0.15cm}{0.15cm}}  7/9 {\tiny (-0.05)} &     \textcolor{red}{\rule{0.15cm}{0.15cm}}  7/10 {\tiny (-0.05)} \\
% Mistral-7B-v0.1   &    \textcolor{pink}{\rule{0.15cm}{0.15cm}}  1/1 {\tiny (-0.02)} &   \textcolor{purple}{\rule{0.15cm}{0.15cm}}  0/2 {\tiny (+0.07)} &   \textcolor{gray}{\rule{0.15cm}{0.15cm}}  3/3 {\tiny (-0.11)} &      \textcolor{red}{\rule{0.15cm}{0.15cm}}  1/4 {\tiny (+0.05)} &  \textcolor{yellow}{\rule{0.15cm}{0.15cm}}  3/5 {\tiny (-0.00)} &    \textcolor{green}{\rule{0.15cm}{0.15cm}}  2/6 {\tiny (+0.02)} &    \textcolor{brown}{\rule{0.15cm}{0.15cm}}  3/7 {\tiny (+0.00)} &    \textcolor{gold}{\rule{0.15cm}{0.15cm}}  7/8 {\tiny (-0.06)} &     \textcolor{blue}{\rule{0.15cm}{0.15cm}}  3/9 {\tiny (+0.03)} &   \textcolor{black}{\rule{0.15cm}{0.15cm}}  5/10 {\tiny (-0.01)} \\
% Mistral-7B-v0.3   &    \textcolor{green}{\rule{0.15cm}{0.15cm}}  0/1 {\tiny (+0.03)} &      \textcolor{red}{\rule{0.15cm}{0.15cm}}  1/2 {\tiny (+0.01)} &  \textcolor{orange}{\rule{0.15cm}{0.15cm}}  2/3 {\tiny (-0.04)} &    \textcolor{pink}{\rule{0.15cm}{0.15cm}}  3/4 {\tiny (-0.04)} &  \textcolor{purple}{\rule{0.15cm}{0.15cm}}  2/5 {\tiny (-0.00)} &   \textcolor{black}{\rule{0.15cm}{0.15cm}}  4/6 {\tiny (-0.04)} &     \textcolor{gold}{\rule{0.15cm}{0.15cm}}  1/7 {\tiny (+0.01)} &  \textcolor{yellow}{\rule{0.15cm}{0.15cm}}  5/8 {\tiny (-0.02)} &     \textcolor{blue}{\rule{0.15cm}{0.15cm}}  2/9 {\tiny (+0.01)} &   \textcolor{brown}{\rule{0.15cm}{0.15cm}}  5/10 {\tiny (-0.01)} \\
% Mixtral-8x7B-v0.1 &   \textcolor{green}{\rule{0.15cm}{0.15cm}}  1/1 {\tiny (-0.10)} &  \textcolor{purple}{\rule{0.15cm}{0.15cm}}  1/2 {\tiny (-0.02)} &     \textcolor{red}{\rule{0.15cm}{0.15cm}}  3/3 {\tiny (-0.04)} &    \textcolor{gold}{\rule{0.15cm}{0.15cm}}  3/4 {\tiny (-0.08)} &   \textcolor{black}{\rule{0.15cm}{0.15cm}}  2/5 {\tiny (-0.03)} &   \textcolor{gray}{\rule{0.15cm}{0.15cm}}  5/6 {\tiny (-0.04)} &  \textcolor{yellow}{\rule{0.15cm}{0.15cm}}  3/7 {\tiny (-0.02)} &   \textcolor{brown}{\rule{0.15cm}{0.15cm}}  6/8 {\tiny (-0.06)} &  \textcolor{orange}{\rule{0.15cm}{0.15cm}}  8/9 {\tiny (-0.06)} &   \textcolor{pink}{\rule{0.15cm}{0.15cm}}  10/10 {\tiny (-0.06)} \\
% Yi-1.5-34B        &    \textcolor{black}{\rule{0.15cm}{0.15cm}}  0/1 {\tiny (+0.01)} &   \textcolor{orange}{\rule{0.15cm}{0.15cm}}  1/2 {\tiny (+0.00)} &   \textcolor{yellow}{\rule{0.15cm}{0.15cm}}  0/3 {\tiny (+0.02)} &     \textcolor{blue}{\rule{0.15cm}{0.15cm}}  0/4 {\tiny (+0.02)} &     \textcolor{gold}{\rule{0.15cm}{0.15cm}}  0/5 {\tiny (+0.04)} &  \textcolor{purple}{\rule{0.15cm}{0.15cm}}  3/6 {\tiny (-0.01)} &   \textcolor{green}{\rule{0.15cm}{0.15cm}}  5/7 {\tiny (-0.04)} &     \textcolor{red}{\rule{0.15cm}{0.15cm}}  8/8 {\tiny (-0.07)} &    \textcolor{pink}{\rule{0.15cm}{0.15cm}}  5/9 {\tiny (-0.04)} &   \textcolor{gray}{\rule{0.15cm}{0.15cm}}  8/10 {\tiny (-0.07)} \\
% Yi-1.5-9B         &  \textcolor{purple}{\rule{0.15cm}{0.15cm}}  0/1 {\tiny (-0.01)} &    \textcolor{blue}{\rule{0.15cm}{0.15cm}}  1/2 {\tiny (-0.01)} &    \textcolor{pink}{\rule{0.15cm}{0.15cm}}  2/3 {\tiny (-0.02)} &  \textcolor{yellow}{\rule{0.15cm}{0.15cm}}  3/4 {\tiny (-0.02)} &     \textcolor{red}{\rule{0.15cm}{0.15cm}}  3/5 {\tiny (-0.04)} &   \textcolor{brown}{\rule{0.15cm}{0.15cm}}  5/6 {\tiny (-0.04)} &    \textcolor{gold}{\rule{0.15cm}{0.15cm}}  2/7 {\tiny (-0.02)} &   \textcolor{gray}{\rule{0.15cm}{0.15cm}}  5/8 {\tiny (-0.04)} &   \textcolor{black}{\rule{0.15cm}{0.15cm}}  6/9 {\tiny (-0.04)} &   \textcolor{green}{\rule{0.15cm}{0.15cm}}  8/10 {\tiny (-0.05)} \\
% gemma-2-27b       &  \textcolor{yellow}{\rule{0.15cm}{0.15cm}}  1/1 {\tiny (-0.04)} &    \textcolor{blue}{\rule{0.15cm}{0.15cm}}  1/2 {\tiny (-0.01)} &  \textcolor{orange}{\rule{0.15cm}{0.15cm}}  2/3 {\tiny (-0.02)} &  \textcolor{purple}{\rule{0.15cm}{0.15cm}}  4/4 {\tiny (-0.03)} &   \textcolor{green}{\rule{0.15cm}{0.15cm}}  4/5 {\tiny (-0.03)} &   \textcolor{black}{\rule{0.15cm}{0.15cm}}  5/6 {\tiny (-0.02)} &     \textcolor{red}{\rule{0.15cm}{0.15cm}}  4/7 {\tiny (-0.02)} &   \textcolor{gray}{\rule{0.15cm}{0.15cm}}  6/8 {\tiny (-0.04)} &    \textcolor{pink}{\rule{0.15cm}{0.15cm}}  8/9 {\tiny (-0.04)} &   \textcolor{gold}{\rule{0.15cm}{0.15cm}}  10/10 {\tiny (-0.05)} \\
% gemma-2-9b        &  \textcolor{purple}{\rule{0.15cm}{0.15cm}}  1/1 {\tiny (-0.09)} &     \textcolor{red}{\rule{0.15cm}{0.15cm}}  2/2 {\tiny (-0.15)} &    \textcolor{pink}{\rule{0.15cm}{0.15cm}}  3/3 {\tiny (-0.14)} &   \textcolor{green}{\rule{0.15cm}{0.15cm}}  4/4 {\tiny (-0.16)} &   \textcolor{brown}{\rule{0.15cm}{0.15cm}}  4/5 {\tiny (-0.14)} &  \textcolor{orange}{\rule{0.15cm}{0.15cm}}  6/6 {\tiny (-0.13)} &  \textcolor{yellow}{\rule{0.15cm}{0.15cm}}  7/7 {\tiny (-0.16)} &    \textcolor{gold}{\rule{0.15cm}{0.15cm}}  8/8 {\tiny (-0.13)} &   \textcolor{black}{\rule{0.15cm}{0.15cm}}  9/9 {\tiny (-0.19)} &  \textcolor{gray}{\rule{0.15cm}{0.15cm}}  10/10 {\tiny (-0.29)} \\
% gpt-3.5           &      \textcolor{red}{\rule{0.15cm}{0.15cm}}  0/1 {\tiny (+0.01)} &  \textcolor{yellow}{\rule{0.15cm}{0.15cm}}  1/2 {\tiny (-0.03)} &  \textcolor{orange}{\rule{0.15cm}{0.15cm}}  3/3 {\tiny (-0.03)} &    \textcolor{pink}{\rule{0.15cm}{0.15cm}}  3/4 {\tiny (-0.04)} &    \textcolor{gold}{\rule{0.15cm}{0.15cm}}  4/5 {\tiny (-0.05)} &    \textcolor{blue}{\rule{0.15cm}{0.15cm}}  3/6 {\tiny (-0.01)} &   \textcolor{brown}{\rule{0.15cm}{0.15cm}}  5/7 {\tiny (-0.03)} &   \textcolor{gray}{\rule{0.15cm}{0.15cm}}  6/8 {\tiny (-0.04)} &   \textcolor{black}{\rule{0.15cm}{0.15cm}}  6/9 {\tiny (-0.02)} &  \textcolor{purple}{\rule{0.15cm}{0.15cm}}  8/10 {\tiny (-0.04)} \\
% gpt-4-turbo       &   \textcolor{brown}{\rule{0.15cm}{0.15cm}}  0/1 {\tiny (-0.01)} &    \textcolor{pink}{\rule{0.15cm}{0.15cm}}  2/2 {\tiny (-0.07)} &    \textcolor{gold}{\rule{0.15cm}{0.15cm}}  3/3 {\tiny (-0.06)} &   \textcolor{green}{\rule{0.15cm}{0.15cm}}  4/4 {\tiny (-0.09)} &  \textcolor{purple}{\rule{0.15cm}{0.15cm}}  4/5 {\tiny (-0.05)} &     \textcolor{red}{\rule{0.15cm}{0.15cm}}  5/6 {\tiny (-0.04)} &   \textcolor{black}{\rule{0.15cm}{0.15cm}}  5/7 {\tiny (-0.01)} &  \textcolor{orange}{\rule{0.15cm}{0.15cm}}  5/8 {\tiny (-0.05)} &    \textcolor{blue}{\rule{0.15cm}{0.15cm}}  6/9 {\tiny (-0.04)} &  \textcolor{yellow}{\rule{0.15cm}{0.15cm}}  7/10 {\tiny (-0.03)} \\
% gpt-4o            &     \textcolor{red}{\rule{0.15cm}{0.15cm}}  1/1 {\tiny (-0.05)} &   \textcolor{green}{\rule{0.15cm}{0.15cm}}  2/2 {\tiny (-0.05)} &  \textcolor{yellow}{\rule{0.15cm}{0.15cm}}  2/3 {\tiny (-0.02)} &  \textcolor{purple}{\rule{0.15cm}{0.15cm}}  3/4 {\tiny (-0.04)} &  \textcolor{orange}{\rule{0.15cm}{0.15cm}}  4/5 {\tiny (-0.03)} &    \textcolor{pink}{\rule{0.15cm}{0.15cm}}  6/6 {\tiny (-0.05)} &   \textcolor{black}{\rule{0.15cm}{0.15cm}}  7/7 {\tiny (-0.04)} &   \textcolor{gray}{\rule{0.15cm}{0.15cm}}  7/8 {\tiny (-0.04)} &   \textcolor{brown}{\rule{0.15cm}{0.15cm}}  9/9 {\tiny (-0.06)} &   \textcolor{gold}{\rule{0.15cm}{0.15cm}}  10/10 {\tiny (-0.06)} \\
% gpt-4o-mini       &  \textcolor{purple}{\rule{0.15cm}{0.15cm}}  0/1 {\tiny (-0.01)} &    \textcolor{pink}{\rule{0.15cm}{0.15cm}}  2/2 {\tiny (-0.06)} &  \textcolor{yellow}{\rule{0.15cm}{0.15cm}}  3/3 {\tiny (-0.03)} &     \textcolor{red}{\rule{0.15cm}{0.15cm}}  3/4 {\tiny (-0.04)} &    \textcolor{blue}{\rule{0.15cm}{0.15cm}}  5/5 {\tiny (-0.07)} &   \textcolor{green}{\rule{0.15cm}{0.15cm}}  6/6 {\tiny (-0.05)} &    \textcolor{gold}{\rule{0.15cm}{0.15cm}}  7/7 {\tiny (-0.07)} &   \textcolor{black}{\rule{0.15cm}{0.15cm}}  8/8 {\tiny (-0.12)} &   \textcolor{brown}{\rule{0.15cm}{0.15cm}}  9/9 {\tiny (-0.13)} &  \textcolor{gray}{\rule{0.15cm}{0.15cm}}  10/10 {\tiny (-0.14)} \\
\bottomrule
\end{tabular}
\caption{\textbf{Color Rankings.} The colors are ranked by the number of colors they \textit{dominate} when listed first. Each cell ${K} / {N} {\tiny ( \pm \bar{\delta}) }$ is the number of colors $K$ whose calibration is statistically significantly less than the calibration when that color is listed first versus second within a prompt. $N$ is the number of colors under that color's rank. $\bar{\delta}$ is the mean change in calibration (WD); larger negative absolute values is a greater effect. The color squares denote the color at that rank for the model of a given row. \textbf{Example:} The cell in the bottom right corner: For gpt-4o-mini, listing white before any of the other 10 colors leads to a statistically significant reduction in WD (improved calibration), with an average performance increase (WD reduction) of -0.14.
\textbf{Takeaways: (1)} There are modest shared preferences across models, with two models having orderings that meaningfully different listed first. \textbf{(2)} While there are significant performance differences among many color pairs the differences are relatively small (notice the mean deltas). \textbf{Average Rank}: For the interested reader, we show the colors in their average rank order (of all models except the first two) though this does not correspond directly to any model's preferences. }
\label{tab:color-rankings}
\end{table*}

==> archive/arr_re.tex <==




\begin{table}[ht!]
\small
\centering

\begin{tabular}{@{}l@{\hspace{4pt}}r@{\hspace{4pt}}c@{\hspace{4pt}}|r@{\hspace{4pt}}c@{\hspace{4pt}}r@{}}
\toprule
{} & \multicolumn{2}{@{}c}{\textit{colors}} & \multicolumn{2}{@{}c}{\textit{wordproblems}} \\
{} &     $\textrm{RE}$ &                              {\scriptsize{(95\% CI)}} &   $\textrm{RE}$  &  {\scriptsize{(95\% CI)}} \\
\midrule
Pick First/Second       &  -0.86 &  {\scriptsize{(-0.88, -0.84)}} &  -0.81 &  {\scriptsize{(-0.82, -0.80)}} \\
Pick $\textrm{Higher}_{p=1.0}$      &  -0.86 &  {\scriptsize{(-0.88, -0.84)}} &  -0.81 &  {\scriptsize{(-0.82, -0.80)}} \\
% pick higher 0.6  &   0.11 &    {\scriptsize{(0.09, 0.13)}} &   0.16 &    {\scriptsize{(0.15, 0.17)}} \\
% pick higher 0.65 &   0.07 &    {\scriptsize{(0.05, 0.09)}} &   0.12 &    {\scriptsize{(0.12, 0.13)}} \\
Pick $\textrm{Higher}_{p=0.7}$    &   0.02 &    {\scriptsize{(0.00, 0.04)}} &   0.07 &    {\scriptsize{(0.06, 0.08)}} \\
% pick higher 0.75 &  -0.05 &  {\scriptsize{(-0.07, -0.03)}} &   0.00 &   {\scriptsize{(-0.01, 0.01)}} \\
% pick higher 0.8  &  -0.14 &  {\scriptsize{(-0.16, -0.12)}} &  -0.09 &  {\scriptsize{(-0.10, -0.08)}} \\
% pick higher 0.85 &  -0.25 &  {\scriptsize{(-0.27, -0.23)}} &  -0.20 &  {\scriptsize{(-0.21, -0.19)}} \\
% pick higher 0.9  &  -0.49 &  {\scriptsize{(-0.50, -0.47)}} &  -0.43 &  {\scriptsize{(-0.44, -0.43)}} \\
Pick Lower       &  -0.86 &  {\scriptsize{(-0.88, -0.84)}} &  -0.81 &  {\scriptsize{(-0.82, -0.80)}} \\
$\textrm{Random}_{\tau=0.01}$    &  -0.83 &  {\scriptsize{(-0.85, -0.80)}} &  -0.77 &  {\scriptsize{(-0.77, -0.76)}} \\
% random-t:0.1     &  -0.48 &  {\scriptsize{(-0.52, -0.44)}} &  -0.42 &  {\scriptsize{(-0.43, -0.41)}} \\
% random-t:1.0     &   0.11 &    {\scriptsize{(0.09, 0.13)}} &   0.16 &    {\scriptsize{(0.15, 0.17)}} \\
% random-t:10.0    &   0.14 &    {\scriptsize{(0.12, 0.16)}} &   0.19 &    {\scriptsize{(0.18, 0.20)}} \\
% random-t:1000.0  &   0.14 &    {\scriptsize{(0.12, 0.16)}} &   0.19 &    {\scriptsize{(0.18, 0.20)}} \\
$\textrm{Random}_{\tau=2}$     &   0.13 &    {\scriptsize{(0.11, 0.15)}} &   0.18 &    {\scriptsize{(0.18, 0.19)}} \\
\midrule
\textit{colors}\\
Meta-Llama-3.1-8B &   0.08$_{\pm0.01}$ &  -0.11$_{\pm0.02}$ \\
Mistral-7B-v0.1   &   0.10$_{\pm0.01}$ &  -0.21$_{\pm0.02}$ \\
Mistral-7B-v0.3   &   0.09$_{\pm0.01}$ &  -0.36$_{\pm0.03}$ \\
Mixtral-8x7B-v0.1 &   0.06$_{\pm0.01}$ &  -0.67$_{\pm0.01}$ \\
Yi-1.5-9B         &   0.06$_{\pm0.02}$ &  -0.55$_{\pm0.01}$ \\
Yi-1.5-34B        &   0.02$_{\pm0.02}$ &  -0.45$_{\pm0.02}$ \\
gemma-2-9b        &   0.13$_{\pm0.01}$ &  -0.44$_{\pm0.01}$ \\
gemma-2-27b       &   0.06$_{\pm0.01}$ &  -0.63$_{\pm0.01}$ \\
gpt-3.5           &                   - &  -0.35$_{\pm0.03}$ \\
gpt-4-turbo       &                   - &  -0.65$_{\pm0.01}$ \\
gpt-4o-mini       &                   - &  -0.53$_{\pm0.01}$ \\
gpt-4o            &                   - &  -0.61$_{\pm0.00}$ \\
\midrule
\textit{wordproblems}\\
Meta-Llama-3.1-8B &  -0.11$_{\pm0.04}$ &  -0.33$_{\pm0.06}$ \\
Mistral-7B-v0.1   &  -0.10$_{\pm0.05}$ &  -0.24$_{\pm0.04}$ \\
Mistral-7B-v0.3   &  -0.12$_{\pm0.05}$ &  -0.47$_{\pm0.04}$ \\
Mixtral-8x7B-v0.1 &  -0.13$_{\pm0.07}$ &  -0.65$_{\pm0.05}$ \\
Yi-1.5-9B         &  -0.11$_{\pm0.05}$ &  -0.55$_{\pm0.03}$ \\
Yi-1.5-34B        &  -0.17$_{\pm0.05}$ &  -0.53$_{\pm0.04}$ \\
gemma-2-9b        &  -0.07$_{\pm0.04}$ &  -0.45$_{\pm0.03}$ \\
gemma-2-27b       &  -0.07$_{\pm0.06}$ &  -0.57$_{\pm0.02}$ \\
gpt-3.5           &                   - &  -0.68$_{\pm0.04}$ \\
gpt-4-turbo       &                   - &  -0.69$_{\pm0.04}$ \\
gpt-4o-mini       &                   - &  -0.58$_{\pm0.05}$ \\
gpt-4o            &                   - &  -0.63$_{\pm0.04}$ \\
\midrule
\textit{distributions}\\
Meta-Llama-3.1-8B &   1.16$_{\pm0.01}$ &   0.69$_{\pm0.01}$ \\
Mistral-7B-v0.1   &   1.12$_{\pm0.01}$ &   1.03$_{\pm0.01}$ \\
Mistral-7B-v0.3   &   1.13$_{\pm0.01}$ &   0.51$_{\pm0.02}$ \\
Mixtral-8x7B-v0.1 &   1.02$_{\pm0.00}$ &   0.26$_{\pm0.02}$ \\
Yi-1.5-9B         &   1.10$_{\pm0.01}$ &   0.48$_{\pm0.02}$ \\
Yi-1.5-34B        &   1.02$_{\pm0.01}$ &   0.38$_{\pm0.02}$ \\
gemma-2-9b        &   1.17$_{\pm0.01}$ &   0.48$_{\pm0.02}$ \\
gemma-2-27b       &   1.05$_{\pm0.00}$ &   0.47$_{\pm0.02}$ \\
gpt-3.5           &                   - &   0.69$_{\pm0.01}$ \\
gpt-4-turbo       &                   - &   0.31$_{\pm0.01}$ \\
gpt-4o-mini       &                   - &   0.41$_{\pm0.01}$ \\
gpt-4o            &                   - &   0.58$_{\pm0.01}$ \\
% Meta-Llama-3.1-8B &  -0.11 &  {\scriptsize{(-0.13, -0.09)}} &  -0.33 &  {\scriptsize{(-0.38, -0.27)}} \\
% Mistral-7B-v0.1   &  -0.21 &  {\scriptsize{(-0.23, -0.19)}} &  -0.24 &  {\scriptsize{(-0.28, -0.20)}} \\
% Mistral-7B-v0.3   &  -0.36 &  {\scriptsize{(-0.39, -0.33)}} &  -0.47 &  {\scriptsize{(-0.51, -0.43)}} \\
% Mixtral-8x7B-v0.1 &  -0.67 &  {\scriptsize{(-0.68, -0.66)}} &  -0.65 &  {\scriptsize{(-0.70, -0.61)}} \\
% Yi-1.5-9B         &  -0.55 &  {\scriptsize{(-0.56, -0.54)}} &  -0.55 &  {\scriptsize{(-0.59, -0.52)}} \\
% Yi-1.5-34B        &  -0.45 &  {\scriptsize{(-0.46, -0.43)}} &  -0.53 &  {\scriptsize{(-0.57, -0.49)}} \\
% gemma-2-9b        &  -0.44 &  {\scriptsize{(-0.45, -0.42)}} &  -0.45 &  {\scriptsize{(-0.48, -0.42)}} \\
% gemma-2-27b       &  -0.63 &  {\scriptsize{(-0.64, -0.62)}} &  -0.57 &  {\scriptsize{(-0.59, -0.55)}} \\
% gpt-3.5           &  -0.35 &  {\scriptsize{(-0.37, -0.32)}} &  -0.68 &  {\scriptsize{(-0.72, -0.64)}} \\
% gpt-4-turbo       &  -0.65 &  {\scriptsize{(-0.66, -0.64)}} &  -0.69 &  {\scriptsize{(-0.73, -0.65)}} \\
% gpt-4o-mini       &  -0.53 &  {\scriptsize{(-0.53, -0.52)}} &  -0.58 &  {\scriptsize{(-0.63, -0.52)}} \\
% gpt-4o            &  -0.61 &  {\scriptsize{(-0.62, -0.61)}} &  -0.63 &  {\scriptsize{(-0.67, -0.59)}} \\
% $\textrm{Random}_{\tau = 0.1}$     &     \multicolumn{2}{c}{1.00} &     \multicolumn{2}{c}{0.50} &  \multicolumn{2}{c}{0.55} \\
% $\texttt{pick higher}_{p = 0.7}$   &     \multicolumn{2}{c}{1.00} &     \multicolumn{2}{c}{1.07} &  \multicolumn{2}{c}{0.15} \\
% $\texttt{pick higher}_{p = 1.0}$        &     \multicolumn{2}{c}{1.00} &     \multicolumn{2}{c}{0.00} &  \multicolumn{2}{c}{0.47} \\
\bottomrule
\end{tabular}


\caption{\textbf{Relative Entropy Results.} Across two datasets, this plot shows the calibration scores (Wasserstein Distance, WD) for chat versions of models along with 95\% confidence intervals. 
% \textbf{Takeaways: (1)} PM for prompted instruction-tuned models is greater than their base counterparts (in statistically significant manner.) (2) gpt-* models have high PM for the \textit{colors} dataset but much lower for the \textit{wordproblems} dataset.
\textbf{Takeaways: (1)} Every model has low entropy relative to the entropy of a calibrated output.
}
\label{tab:results:re}
\end{table}









==> archive/arr_re_2.tex <==
\begin{table*}[ht!]
\small
\centering
\begin{tabular}{@{}lrr|ll|ll@{}}
\toprule
                            &   \multicolumn{2}{c}{\textit{colors}} &                   \multicolumn{2}{c}{\textit{wordproblems}}        &               \multicolumn{2}{c}{\textit{distributions}}                 \\
\midrule
Pick Higher      &  \multicolumn{2}{c|}{-0.86$_{\pm0.01}$} &  \multicolumn{2}{c|}{-0.81$_{\pm0.00}$} &                                 \multicolumn{2}{c}{-} \\
% pick higher 0.6  &   \multicolumn{2}{c}{0.11$_{\pm0.01}$} &   \multicolumn{2}{c}{0.16$_{\pm0.00}$} &                                 \multicolumn{2}{c}{-} \\
% pick higher 0.65 &   \multicolumn{2}{c}{0.07$_{\pm0.01}$} &   \multicolumn{2}{c}{0.12$_{\pm0.00}$} &                                 \multicolumn{2}{c}{-} \\
Pick $\textrm{Higher}_\textrm{p=0.7}$ &   \multicolumn{2}{c|}{0.02$_{\pm0.01}$} &   \multicolumn{2}{c|}{0.07$_{\pm0.00}$} &                                 \multicolumn{2}{c}{-} \\
% pick higher 0.75 &  \multicolumn{2}{c|}{-0.05$_{\pm0.01}$} &   \multicolumn{2}{c|}{0.00$_{\pm0.00}$} &                                 \multicolumn{2}{c|}{-} \\
% pick higher 0.8  &  \multicolumn{2}{c|}{-0.14$_{\pm0.01}$} &  \multicolumn{2}{c|}{-0.09$_{\pm0.00}$} &                                 \multicolumn{2}{c|}{-} \\
% pick higher 0.85 &  \multicolumn{2}{c|}{-0.25$_{\pm0.01}$} &  \multicolumn{2}{c|}{-0.20$_{\pm0.00}$} &                                 \multicolumn{2}{c|}{-} \\
% pick higher 0.9  &  \multicolumn{2}{c|}{-0.49$_{\pm0.01}$} &  \multicolumn{2}{c|}{-0.43$_{\pm0.00}$} &                                 \multicolumn{2}{c|}{-} \\
Pick Lower       &  \multicolumn{2}{c|}{-0.86$_{\pm0.01}$} &  \multicolumn{2}{c|}{-0.81$_{\pm0.00}$} &                                 \multicolumn{2}{c}{-} \\
Pick First/Second      &  \multicolumn{2}{c|}{-0.86$_{\pm0.01}$} &  \multicolumn{2}{c|}{-0.81$_{\pm0.00}$} &                                 \multicolumn{2}{c}{-} \\
% Pick First       &  \multicolumn{2}{c|}{-0.86$_{\pm0.01}$} &  \multicolumn{2}{c|}{-0.81$_{\pm0.00}$} &                                \multicolumn{2}{c|}{1.66$_{\pm0.01}$}  \\
$\textrm{Random}_{\tau = 0.01}$     &  \multicolumn{2}{c|}{-0.80$_{\pm0.01}$} &  \multicolumn{2}{c|}{-0.76$_{\pm0.00}$} &  \multicolumn{2}{c}{0.11$_{\pm0.01}$} \\
% random-t:0.1     &  \multicolumn{2}{c|}{-0.49$_{\pm0.02}$} &  \multicolumn{2}{c|}{-0.42$_{\pm0.01}$} &  \multicolumn{2}{c|}{0.33$_{\pm0.01}$} \\
$\textrm{Random}_{\tau = 1.0}$     &   \multicolumn{2}{c|}{0.11$_{\pm0.01}$} &   \multicolumn{2}{c|}{0.16$_{\pm0.00}$} &  \multicolumn{2}{c}{1.66$_{\pm0.01}$} \\
% random-t:10.0    &   \multicolumn{2}{c|}{0.14$_{\pm0.01}$} &   \multicolumn{2}{c|}{0.19$_{\pm0.00}$} &                                 \multicolumn{2}{c}{-} \\
% random-t:1000.0  &   \multicolumn{2}{c}{0.14$_{\pm0.01}$} &   \multicolumn{2}{c}{0.19$_{\pm0.00}$} &                                 \multicolumn{2}{c}{-} \\
% random-t:2.0     &   \multicolumn{2}{c}{0.13$_{\pm0.01}$} &   \multicolumn{2}{c}{0.18$_{\pm0.00}$} &                                 \multicolumn{2}{c}{-} \\
\midrule
Meta-Llama-3.1-8B & 0.08$_{\pm0.01}$ & -0.11$_{\pm0.02}$ & -0.11$_{\pm0.04}$ & -0.33$_{\pm0.06}$ & 1.16$_{\pm0.01}$ & 0.69$_{\pm0.01}$ \\
  Mistral-7B-v0.1 & 0.10$_{\pm0.01}$ & -0.21$_{\pm0.02}$ & -0.10$_{\pm0.05}$ & -0.24$_{\pm0.04}$ & 1.12$_{\pm0.01}$ & 1.03$_{\pm0.01}$ \\
  Mistral-7B-v0.3 & 0.09$_{\pm0.01}$ & -0.36$_{\pm0.03}$ & -0.12$_{\pm0.05}$ & -0.47$_{\pm0.04}$ & 1.13$_{\pm0.01}$ & 0.51$_{\pm0.02}$ \\
Mixtral-8x7B-v0.1 & 0.06$_{\pm0.01}$ & -0.67$_{\pm0.01}$ & -0.13$_{\pm0.07}$ & -0.65$_{\pm0.05}$ & 1.02$_{\pm0.00}$ & 0.26$_{\pm0.02}$ \\
       Yi-1.5-34B & 0.02$_{\pm0.02}$ & -0.45$_{\pm0.02}$ & -0.17$_{\pm0.05}$ & -0.53$_{\pm0.04}$ & 1.02$_{\pm0.01}$ & 0.38$_{\pm0.02}$ \\
        Yi-1.5-9B & 0.06$_{\pm0.02}$ & -0.55$_{\pm0.01}$ & -0.11$_{\pm0.05}$ & -0.55$_{\pm0.03}$ & 1.10$_{\pm0.01}$ & 0.48$_{\pm0.02}$ \\
      gemma-2-27b & 0.06$_{\pm0.01}$ & -0.63$_{\pm0.01}$ & -0.07$_{\pm0.06}$ & -0.57$_{\pm0.02}$ & 1.05$_{\pm0.00}$ & 0.47$_{\pm0.02}$ \\
       gemma-2-9b & 0.13$_{\pm0.01}$ & -0.44$_{\pm0.01}$ & -0.07$_{\pm0.04}$ & -0.45$_{\pm0.03}$ & 1.17$_{\pm0.01}$ & 0.48$_{\pm0.02}$ \\
          gpt-3.5 &                 - & -0.35$_{\pm0.03}$ &                  - & -0.68$_{\pm0.04}$ &                 - & 0.69$_{\pm0.01}$ \\
      gpt-4-turbo &                 - & -0.65$_{\pm0.01}$ &                  - & -0.69$_{\pm0.04}$ &                 - & 0.31$_{\pm0.01}$ \\
           gpt-4o &                 - & -0.61$_{\pm0.00}$ &                  - & -0.63$_{\pm0.04}$ &                 - & 0.58$_{\pm0.01}$ \\
      gpt-4o-mini &                 - & -0.53$_{\pm0.01}$ &                  - & -0.58$_{\pm0.05}$ &                 - & 0.41$_{\pm0.01}$ \\
\bottomrule
\end{tabular}

\caption{\textbf{Relative Entropy Results.} Across two datasets, this plot shows the calibration scores (Wasserstein Distance, WD) for chat versions of models along with 95\% confidence intervals. 
% \textbf{Takeaways: (1)} PM for prompted instruction-tuned models is greater than their base counterparts (in statistically significant manner.) (2) gpt-* models have high PM for the \textit{colors} dataset but much lower for the \textit{wordproblems} dataset.
\textbf{Takeaways: (1)} Every model has low entropy relative to the entropy of a calibrated output.
}
\label{tab:results:re}
\end{table*}

==> archive/arr_wd.tex <==
\begin{table}[ht!]
\small
\centering



% % \begin{tabular}{@{}l@{\hspace{4pt}}l@{\hspace{4pt}}r@{\hspace{4pt}}l@{\hspace{4pt}}r@{\hspace{4pt}}r@{}}
% \toprule

% Probability Mass (PM) &  Base &     {\scriptsize{(95\% CI)}} &  Chat &   {\scriptsize{(95\% CI)}} \\
% \midrule
% Idealized &  1.00 & - &  1.00 & - \\
% \midrule
% \textit{colors}\\

\begin{tabular}
{@{}l@{\hspace{4pt}}l@{\hspace{4pt}}c@{\hspace{4pt}}|l@{\hspace{4pt}}c@{\hspace{4pt}}r@{}}
\toprule
{} & \multicolumn{2}{@{}c}{\textit{colors}} & \multicolumn{2}{c}{\textit{wordproblems}} \\
 &     {$\textrm{WD}_\downarrow$} &                              {\scriptsize{(95\% CI)}} &    {$\textrm{WD}_\downarrow$} &  {\scriptsize{(95\% CI)}} \\
\midrule
Pick Lower       &  0.95 &  {\scriptsize{(0.93, 0.97)}} &  0.98 &  {\scriptsize{(0.97, 0.98)}} \\
$\textrm{Random}_{\tau = 0.01}$     &  0.72 &  {\scriptsize{(0.69, 0.76)}} &  0.69 &  {\scriptsize{(0.68, 0.70)}} \\
Pick First/Second       &  0.71 &  {\scriptsize{(0.67, 0.74)}} &  0.71 &  {\scriptsize{(0.70, 0.72)}} \\
Pick $\textrm{Higher}_{p = 1.0}$\spade      &  0.47 &  {\scriptsize{(0.45, 0.49)}} &  0.44 &  {\scriptsize{(0.43, 0.44)}} \\
$\textrm{Random}_{\tau = 2}$     &  0.24 &  {\scriptsize{(0.22, 0.26)}} &  0.28 &  {\scriptsize{(0.27, 0.28)}} \\
Pick $\textrm{Higher}_{p = 0.7}$  &  0.15 &  {\scriptsize{(0.14, 0.16)}} &  0.17 &  {\scriptsize{(0.17, 0.18)}} \\
Idealized &  0.00 & -  & 0.00  & - \\
\midrule
Meta-Llama-3.1-8B &  0.40\spade &  {\scriptsize{(0.39, 0.41)}} &  0.48 &   {\scriptsize{(0.46, 0.50)}} \\
Mistral-7B-v0.1   &  0.50 &  {\scriptsize{(0.49, 0.51)}} &  0.49 &   {\scriptsize{(0.48, 0.50)}} \\
Mistral-7B-v0.3   &  0.48 &  {\scriptsize{(0.46, 0.49)}} &  0.55 &  {\scriptsize{(0.54, 0.56)}} \\
Mixtral-8x7B-v0.1 &  0.51 &   {\scriptsize{(0.50, 0.52)}} &  0.60 &  {\scriptsize{(0.57, 0.63)}} \\
Yi-1.5-9B         &  0.49 &   {\scriptsize{(0.48, 0.50)}} &  0.56 &  {\scriptsize{(0.55, 0.57)}} \\
Yi-1.5-34B        &  0.55 &  {\scriptsize{(0.54, 0.56)}} &  0.57 &  {\scriptsize{(0.55, 0.58)}} \\
gemma-2-9b        &  0.50 &   {\scriptsize{(0.50, 0.51)}} &  0.52 &   {\scriptsize{(0.50, 0.54)}} \\
gemma-2-27b       &  0.40\spade &    {\scriptsize{(0.40, 0.40)}} &  0.48 &  {\scriptsize{(0.47, 0.49)}} \\
gpt-3.5           &  0.30\spade &  {\scriptsize{(0.29, 0.31)}} &  0.57 &  {\scriptsize{(0.55, 0.59)}} \\
gpt-4-turbo       &  0.42\spade &  {\scriptsize{(0.41, 0.43)}} &  0.62 &  {\scriptsize{(0.59, 0.64)}} \\
gpt-4o-mini       &  0.40\spade &   {\scriptsize{(0.39, 0.40)}} &  0.57 &  {\scriptsize{(0.55, 0.59)}} \\
gpt-4o            &  0.40\spade &   {\scriptsize{(0.39, 0.40)}} &  0.57 &  {\scriptsize{(0.56, 0.59)}} \\
\midrule
\bottomrule
\end{tabular}


\caption{\textbf{Calibration Results.} Across two datasets, this plot shows the calibration scores (wasserstein distance, WD) for chat versions of models along with 95\% confidence intervals. For \textit{colors}, six models have a statistically better calibration than the baseline of always picking the option associated with the higher number, denoted \spade. For \textit{wordproblems}, no model is better than this simple baseline.
% \textbf{Takeaways: (1)} PM for prompted instruction-tuned models is greater than their base counterparts (in statistically significant manner.) (2) gpt-* models have high PM for the \textit{colors} dataset but much lower for the \textit{wordproblems} dataset.
}
\label{tab:results:wd}
\end{table}

==> archive/baselines.tex <==
\begin{table}[ht!]
\small
\centering
\begin{tabular}{lrrrrrr}
\toprule
% {} & \multicolumn{2}{c}{Rel. Entropy $\updownarrow$} & \multicolumn{2}{c}{Prob. (PM) $\uparrow$} & \multicolumn{2}{c}{Calibr. (WD) $\downarrow$} \\
{} & \multicolumn{2}{c}{$\textrm{RE}_\updownarrow$} & \multicolumn{2}{c}{$\textrm{PM}_\uparrow$} & \multicolumn{2}{c}{$\textrm{WD}_\downarrow$}\\
\midrule
Idealized & \multicolumn{2}{c}{1.00} & \multicolumn{2}{c}{1.00} & \multicolumn{2}{c}{0.00} \\
$\textrm{Random}_{\tau = 0.01}$     &     \multicolumn{2}{c}{0.10} &    \multicolumn{2}{c}{1.00} &  \multicolumn{2}{c}{0.86} \\
$\textrm{Random}_{\tau = 0.1}$      &   \multicolumn{2}{c}{0.31} &    \multicolumn{2}{c}{1.00} &     \multicolumn{2}{c}{0.78}\\
$\textrm{Random}_{\tau = 1.0}$      &    \multicolumn{2}{c}{1.61} &   \multicolumn{2}{c}{1.00} &   \multicolumn{2}{c}{0.38} \\
\bottomrule
\end{tabular}
\caption{\textbf{Baselines on \texttt{Distributions} Results.} }
\label{tab:baselines:dist}
\end{table}
\begin{table}[ht!]
\small
\centering
\begin{tabular}{lrrrrrr}
\toprule
% {} & \multicolumn{2}{c}{Rel. Entropy $\updownarrow$} & \multicolumn{2}{c}{Prob. (PM) $\uparrow$} & \multicolumn{2}{c}{Calibr. (WD) $\downarrow$} \\
{} & \multicolumn{2}{c}{$\textrm{PM}_\uparrow$} &  \multicolumn{2}{c}{$\textrm{RE}_\updownarrow$} & \multicolumn{2}{c}{$\textrm{WD}_\downarrow$}\\
\midrule
Idealized &  \multicolumn{2}{c}{1.00}  & \multicolumn{2}{c}{1.00}  &  \multicolumn{2}{c}{0.00} \\
\midrule
% $\textrm{Random}_{\tau = 0.01}$     &        \multicolumn{2}{c}{0.06} &       \multicolumn{2}{c}{1.00} &       \multicolumn{2}{c}{0.69} \\
% $\textrm{Random}_{\tau = 0.1}$     &  \multicolumn{2}{c}{0.48} &   \multicolumn{2}{c}{1.00} &    \multicolumn{2}{c}{0.56} \\
% $\textrm{Random}_{\tau = 1.0}$       &   \multicolumn{2}{c}{1.17} &   \multicolumn{2}{c}{1.00} &   \multicolumn{2}{c}{0.27} \\
% $\texttt{pick higher}_{p = 0.6}$  &               \multicolumn{2}{c}{1.18} &      \multicolumn{2}{c}{1.00} &            \multicolumn{2}{c}{0.16} \\
% $\texttt{pick higher}_{p = 0.7}$   &               \multicolumn{2}{c}{1.07} &      \multicolumn{2}{c}{1.00} &            \multicolumn{2}{c}{0.15} \\
% $\texttt{pick higher}_{p = 0.75}$  &               \multicolumn{2}{c}{0.98} &      \multicolumn{2}{c}{1.00} &            \multicolumn{2}{c}{0.18} \\
% $\texttt{pick higher}_{p = 0.8}$    &               \multicolumn{2}{c}{0.87} &      \multicolumn{2}{c}{1.00} &            \multicolumn{2}{c}{0.21} \\
% $\texttt{pick higher}_{p = 0.9}$    &               \multicolumn{2}{c}{0.57} &      \multicolumn{2}{c}{1.00} &            \multicolumn{2}{c}{0.33} \\
% $\texttt{pick higher}_{p = 1.0}$       &               \multicolumn{2}{c}{0.00} &      \multicolumn{2}{c}{1.00} &            \multicolumn{2}{c}{0.46} \\
% $\texttt{pick lower}_{p = 1.0}$        &               \multicolumn{2}{c}{0.00} &      \multicolumn{2}{c}{1.00} &            \multicolumn{2}{c}{0.95} \\
% $\texttt{pick first}_{p = 1.0}$       &               \multicolumn{2}{c}{0.00} &      \multicolumn{2}{c}{1.00} &            \multicolumn{2}{c}{0.70} \\
% $\texttt{pick second}_{p = 1.0}$      &               \multicolumn{2}{c}{0.00} &      \multicolumn{2}{c}{1.00} &            \multicolumn{2}{c}{0.71} \\
% \midrule
$\texttt{pick first}_{p = 1.0}$       &     \multicolumn{2}{c}{1.00} &              \multicolumn{2}{c}{0.00} &           \multicolumn{2}{c}{0.71} \\
$\texttt{pick second}_{p = 1.0}$       &     \multicolumn{2}{c}{1.00} &              \multicolumn{2}{c}{0.00} &           \multicolumn{2}{c}{0.71} \\
\midrule
$\texttt{pick higher}_{p = 0.6}$   &     \multicolumn{2}{c}{1.00} &              \multicolumn{2}{c}{1.17} &           \multicolumn{2}{c}{0.16} \\
$\texttt{pick higher}_{p = 0.65}$   &  \multicolumn{2}{c}{1.00} &              \multicolumn{2}{c}{1.13} &           \multicolumn{2}{c}{0.15} \\
$\texttt{pick higher}_{p = 0.7}$   &     \multicolumn{2}{c}{1.00} &              \multicolumn{2}{c}{1.07} &           \multicolumn{2}{c}{0.15} \\
$\texttt{pick higher}_{p = 0.75}$  &     \multicolumn{2}{c}{1.00} &              \multicolumn{2}{c}{0.98} &           \multicolumn{2}{c}{0.18} \\
$\texttt{pick higher}_{p = 0.8}$    &     \multicolumn{2}{c}{1.00} &              \multicolumn{2}{c}{0.87} &           \multicolumn{2}{c}{0.21} \\
$\texttt{pick higher}_{p = 0.85}$   &     \multicolumn{2}{c}{1.00} &              \multicolumn{2}{c}{0.74} &           \multicolumn{2}{c}{0.26} \\
$\texttt{pick higher}_{p = 0.90}$   &     \multicolumn{2}{c}{1.00} &              \multicolumn{2}{c}{0.46} &           \multicolumn{2}{c}{0.36} \\
$\texttt{pick higher}_{p = 1.0}$        &     \multicolumn{2}{c}{1.00} &              \multicolumn{2}{c}{0.00} &           \multicolumn{2}{c}{0.47} \\
$\texttt{pick lower}_{p = 1.0}$         &     \multicolumn{2}{c}{1.00} &              \multicolumn{2}{c}{0.00} &           \multicolumn{2}{c}{0.95} \\
\midrule
$\textrm{Random}_{\tau = 0.01}$    &     \multicolumn{2}{c}{1.00} &              \multicolumn{2}{c}{0.06} &           \multicolumn{2}{c}{0.69} \\
$\textrm{Random}_{\tau = 0.1}$     &     \multicolumn{2}{c}{1.00} &              \multicolumn{2}{c}{0.50} &           \multicolumn{2}{c}{0.55} \\
$\textrm{Random}_{\tau = 1.0}$       &     \multicolumn{2}{c}{1.00} &              \multicolumn{2}{c}{1.17} &           \multicolumn{2}{c}{0.26} \\
$\textrm{Random}_{\tau = 2.0}$       &     \multicolumn{2}{c}{1.00} &              \multicolumn{2}{c}{1.20} &           \multicolumn{2}{c}{0.25} \\
$\textrm{Random}_{\tau = 10.0}$     &     \multicolumn{2}{c}{1.00} &              \multicolumn{2}{c}{1.21}  &  \multicolumn{2}{c}{0.24} \\         \bottomrule
\end{tabular}
\caption{\textbf{Baseline \texttt{Probabilities} Results.} }
\label{tab:baselines:prob}
\end{table}




==> archive/deprecated_main.tex <==
\section{Introduction}
We investigate if language model (LM) outputs are calibrated to the numeric content of their contexts. Consider the context below:
\begin{exe}
 % \ex \label{intro:example1} {From \textbf{17} \textcolor{blue}{\textit{blue}}  marbles and \textbf{99} \textcolor{red}{\textit{red}} marbles, Tommy reached blindly into a bag and grabbed a marble the color $[blue/red]$} 
 \ex \label{intro:example1b} {From \textbf{98} \textcolor{blue}{\textit{blue}}  marbles and \textbf{99} \textcolor{red}{\textit{red}} marbles, Tommy reached blindly into a bag and grabbed a marble the color $[blue/red]$} 
 \end{exe}
To make this standard concrete, we explore the position that the probabilities for the next generated token should be calibrated to the relevant numeric content. E.g., in the examples above, the probability that an LM continues with the \textit{bracketed tokens} should be proportional to the respective \textbf{bolded} values. In this work, to simplify our experiments, we set aside phenomena like hyperbole and pragmatism, and multiple token words.
% In Example \ref{intro:example1}, the probability of \textit{blue} should be approximately $\frac{1}{5}$th the probability of  \textit{red}. 


\begin{figure}[h]
 \centering
 \includegraphics[width=\linewidth]{figures-keynote/the-medium-fig-arr.pdf}
 \caption{\textbf{Models produce un-calibrated results}. %Inputting Examples 1 and 2 to \texttt{gpt-4o} different, uncalibrated behaviors arise in the model probabilities. For {(1)}, \texttt{gpt-4o} over-weights the first option listed in the prompt, predicting \textcolor{blue}{\textit{blue}} with 90.4\% when 15\% is appropriate. For {(2)},
 \texttt{gpt-4o} over-weights the option with a higher number beyond the calibrated ratio, predicting \textcolor{red}{\textit{red}} with 99.7\% when 50.2\% is appropriate. 
 %We term the first behavior \texttt{Pick First} and the second \texttt{Pick Higher}.
 }
 \label{fig:big-fig}
\end{figure}

\begin{dmbox}{What Do We Mean By Calibration?}
LMs' output probabilities are \textit{calibrated} to their contexts if the probabilities of relevant tokens correspond to the numeric content implicitly or explicitly defined by their contexts. If tokens $t_1, t_2, \dots, t_n$ are indicated by context $C$ to have probabilities $P = p_1, p_2, \dots, p_n$, a calibrated LM $m$ outputs corresponding probabilities $\pi_i = m(t_i | c)$: 
 \[ p_i \propto	 \pi_i,\quad i\- \in \- 
 1, 2, \dots, n. \]
We set calibration as the distance between $P$ and $\Pi = \pi_1, \pi_2, \dots, \pi_n$ (\Cref{sec:design:metrics}).
\end{dmbox}

This work makes and then tests the normative assumption that model probabilities for the next generated token should be calibrated to the relevant numeric content. The idea being that if the context defines or implies a probability to hold true within the context, then subsequent text generation should condition on that probability. Naturally, this raises questions, likr, is this standard actually desirable? Is this a reasonable thing to expect from models? % This paper focuses on where and how models deviate from this high standard, but for now we want to highlight why this standard is a good idea.

Numerically calibrated results may be unreasonable to expect from current models, especially given how pre-training datasets are constructed. \cite{zhou-etal-2023-navigating} highlight how different numbers appear with different frequencies and, presumably, in different contexts.
\noindent The numbers 98 and 99 may be used differently across the pre-training corpus, so expecting outputs dependent on those numbers to be similarly calibrated may be a tall order.  Similarly, models' mathematical capabilities have long lagged behind other capabilities and, as such, receive careful attention \citep{mathstral2025}. From this point of view, numeric calibration may look like considering only a sub-case of a larger, known problem. For two primary reasons we believe it is worth studying. Models are now much better at mathematical reasoning, capabilities are improving significantly \citep{lin2024rho,shao2024deepseekmath}. 
Calibration, while tied to mathematical understanding, may  not improve as the general mathematical capabilities of models improve, and some of the fixes may not transfer well to calibration \citep{singh2024tokenization}. Moreover, this failure mode, not reaching this standard of calibration, is not necessarily obvious from the perspective of a single user. Patterns of failed calibration may only be impact a population as a whole. %, but that does not mean pre-emptively trying to capture this failure mode is unimportant.

Models are mostly trained on natural outputs from human data, and people are often biased making it more difficult for models to arrive at calibrated behavior. But the design decisions about how models are trained should not bear on the behavior we would like models to have. Uncalibrated models can impact users via uncalibrated recommendations between, say, different restaurants, vacation options, or candidate employees. Although these options are not obviously tied to numeric values, there is some underlying weighting tied between options and recommendations. We focus on a simplified setting where numeric values are surfaced and calibrated behavior is unambiguous.
% All that being said, people use these models and if they are uncalibrated this will impact their use.


% We also evaluated how models behave when prompted to sample from distributions, like below:
% % \setcounter{ex}{2}
% \begin{exe}
%  \ex \label{intro:example2} {Sampling from a uniform distribution with support from \textbf{2} inclusive to \textbf{5} exclusive, I sampled the number $[\textit{0}/\textit{1}/\textit{2}/\textit{3}\dots\textit{9}]$}
% \end{exe}
% In Example \ref{intro:example2}, the tokens \textit{2, 3, 4} should each have a probability of $\sfrac{1}{3}$, while other digits should have probabilities close to 0. In sum, when the desired output is dependent on probabilities discernible from the context, randomness should arise from the model probabilities and the sampling algorithm, rather than from other arbitrary factors.å

Stepping back, our motivation is drawn from the fact that while pre-training endows language models with a wide range of capabilities \citep{brown2020language, wei2022emergent}, further training can increase the utility of existing models by encouraging them to follow instructions \citep{wei2021finetuned,sanh2021multitask} or match human preferences \citep{ouyang2022training} rather than human behavior implicit in natural human text. Ideally, a model's overt reasoning process aligns with its internal reasoning process \citep{lanham2023measuring}. This idea underlies some model explanation methods \citep{chen2023models}: counterfactual simulatability requires that an explanation captures the ``reason'' a model arrived at an answer. Along the same lines, for contexts that call for contextual calibration, e.g., situations where the context suggests probabilities over the next tokens,  the most direct solution is for models to yield exactly those probabilities. \citet{kusner2017counterfactual} also studies probability differences in the setting of counterfactual fairness.

There are large-scale efforts for models to not reproduce endemic online biases \citep{bai2022training,rudinger2018}; we test if models are calibrated to the numeric content in context rather than other patterns. Such biases are common with people, like the first-mentioned bias \citep{van2024random} where the first option listed is favored. LLMs have also been shown to exhibit biases concerning option order in multiple-choice questions \citep{pezeshkpour-hruschka-2024-large}.


\begin{dmbox}{Contributions: Models Are \textit{Not} Calibrated}
Though different models have different error patterns, no model is well-calibrated. %Moreover, there are some shared themes across models and model families:
\begin{enumerate}[leftmargin=*]
 \item Mode collapse: Instruction-tuning tends to improve the allocation of probability mass upon valid options, but instruction-tuning also leads to decreased entropy in model outputs. This can both improve (such as in Example \ref{intro:example1}) or reduce (such as in Example \ref{intro:example2}) calibration.
 \item Models have systematic tendencies: Many models show preferences for certain tokens (such as numbers or colors), and the word order can also influence which tokens the models favor.
\end{enumerate}
\end{dmbox}

\section{Related Work}
\paragraph{Models struggle to calibrate internal uncertainty with textual outputs.} 
A related but separate line of work studies how well models calibrate their prediction confidence with prediction accuracy: a calibrated model with $0.80$ confidence on each prediction should classify $80\%$ of examples correctly \citep{guo2017calibration, minderer2021revisiting}. Another line of work investigates how well model outputs align with uncertainty \citep{yona2024can,kumar2024confidence,zhou-etal-2023-navigating,lin2022teaching}, termed linguistic calibration \citep{mielke2022reducing}. \citet{yona2024can} report that models struggle to exhibit internal uncertainty in text; \citet{kumar2024confidence} measures how well confidence is aligned internally (model probabilities) and externally (via eliciting model to choose among a Likert scale.) In our work, we look the agreement between the probability of predicted outputs and the contextually defined likelihood of outputs in the text. We find that models often are \textit{certain} when they should be \textit{uncertain}; {mode collapse} arises both via supervised fine-tuning and reward-based fine-tuning \citep{oattributing, janus2024modecollapse}. \citet{zhou-etal-2024-relying} also finds that RLHF biases models towards certainty, over generating strengtheners (e.g., ``I am certain\dots'') over weakeners  (e.g., ``Maybe\dots'').

%Reward Modeling Is Biased Towards Certainty to over-generate strengtheners (e.g., ``I am certain\dots''), 

% \citep{zhou-etal-2024-relying}

\paragraph{Recent work investigates if language models can output random results.} \citet{van2024random} shows that single coin flip predictions are biased towards heads and a first-mentioned bias. \citet{silva2024large} shows that large models can 1) correctly describe Matching Pennies, a popular game in game theory, and 2) code optimal behavior. \citet{hopkins2023can}, work closely related to our own, examines whether LMs can induce uniform distributions in the 0 to 1 interval. 

\section{Experimental Design}\label{sec:design}
We design two experiments to evaluate whether model probabilities calibrate to contextual numeric information, \Cref{sec:exp:exp1} and \Cref{sec:exp:exp2}.\footnote{See \Cref{app:details} for reproducibility.}

\subsection{Problem Setup}\label{sec:design:problem_setup}
Each problem is defined as a context $C$ to be continued by a relevant token among $t_1, t_2, \dots, t_n = T \subset V$, where $V$ is the full vocabulary. Each token $t_i$ is associated with a probability $p_i$ forming a distribution, $P = p_1, p_2, \dots, p_n$. In Example \ref{intro:example2}, $T$ is $\{\textrm{\textit{red}}, \textrm{\textit{blue}}\}$ with $P = \{\textrm{\textit{red}} : \sfrac{98}{197}, \textrm{\textit{blue}} : \sfrac{99}{197}\}$. For a model $m$, we define $\Pi = \pi_1, \pi_2, \dots$ where $\pi_i \approx m(t_i | C)$, with one addendum. We sum the probabilities of all common tokenizations for a given word, including capitalization and spaces: $\pi_i = \sum_{s \in \textrm{Tokenizations}(t_i)} m(s | C)$. E.g., we sum probabilities for ``red'', ``Red'', ``\_red'', and ``\_Red.'' This approach to the problem of there being many reasonable continuations to even our constrained contexts is imperfect, but informally works quite well in capturing the model's valid outputs. Empirically, the high PM values (near 1) support this conclusion. Notably, this is less true for our second experiment, \cref{sec:exp:exp2}.

\subsection{Metrics and Evaluation}\label{sec:design:metrics}
Our primary metrics below help us ask how well a model calibrates to numeric information in context.

\textbf{Probability Mass (PM)}: Calibration, the relative probability mass across tokens in \textit{T}, is well-founded if the \textbf{PM} over $T$ is sufficiently large, 
$\textrm{PM}(T) \doteq \sum_{t\,:\,T} \pi_t
.$
If $\textrm{PM}(T)$ for a model is low (say, 0.30), then it is  unclear if the model is capturing the intended relationship between the context and $T$. However, when $\textrm{PM}$ is high (say, 0.75), we can start to meaningfully ask questions about how probability mass is allocated among, say, \textit{red} and \textit{blue}. Our metric for measuring calibration (introduced below) would also capture when the PM is too low, but also separately measuring the PM makes it easier to understand the results.

\textbf{Relative Entropy (RE):} To detect mode collapse, we measure \textbf{RE}, the ratio between entropy $\textrm{H}$ of model probabilities and calibrated probabilities, $\textrm{H}(\Pi)/\textrm{H}(P)$. An $\textrm{RE} < 1$ means that the probability mass is overly concentrated.
 
\textbf{Wasserstein Distance (WD)}: To measure  \textbf{calibration}, we use \textbf{WD}. 
WD \citep{kantorovich1939mathematical}
 captures the movement between one distribution (or set of values) and another.\footnote{Kullback–Leibler (KL) divergence is also a natural choice. However, a number of the target distributions we have include 0 values where KL would be undefined. We also compute Mean-Squared Error (MSE) but don't find a material difference in the findings so only report the WD.} %

\subsection{Models} We test open-source models that have both base and instruction-tuned versions: \texttt{Mistral-7B-v0.1}, \texttt{Mistral-7B-v0.3}, \texttt{Mixtral-8x7B-v0.1}, \texttt{Yi-1.5-9B}, \texttt{Yi-1.5-34B}, \texttt{Meta-Llama-3.1-8B}, \texttt{gemma-2-9b}, \texttt{gemma-2-27b} \citep{jiang2023mistral,jiang2024mixtral,young2024yi,dubey2024llama,team2024gemma}; and four proprietary models, \texttt{gpt-3.5}, \texttt{gpt-4-turbo}, \texttt{gpt-4o-mini}, and \texttt{gpt-4o} \citep{brown2020language,achiam2023gpt,openai2023gpt4o}. We prompt instruction-tuned models to be calibrated. We refer to the base, unprompted version of the models as ``base'' and the instruction-tuned, prompted models as ``chat.'' % Model keys are listed in Appendix \Cref{tab:models}.
        
\subsection{Experiment: \texttt{Distributions}}\label{sec:exp:exp1}
This experiment tests if models can generate relevant tokens uniformly. Example \ref{intro:example2} is representative of the dataset: 
\begin{exe}    
\ex \label{intro:example2}
 {Sampling from a uniform distribution with support from \textbf{2} inclusive to \textbf{5} exclusive, I sampled the number $[\textit{0}/\textit{1}/\textit{2}/\textit{3}\dots\textit{9}]$}
\end{exe}
We test across different numeric ranges, range inclusivities, and templates. The numbers scale from 10 to 1000 and we use 5 different templates; there are 4500 unique instances. In some of our analyses, we group problems that support the same tokens: For example, [12, 15) and [92, 95) are grouped together. There are 615 such groups.

The question is if the distribution of the next token is calibrated to the uniform distribution $\Pi^C = \mathcal{U}(2, 5)$. As noted above, we report WD, which for this example would be: $\textrm{WD}(\Pi^T, \mathcal{U}(2, 5)) = \textrm{WD}(\Pi^T, [0, 0, \sfrac{1}{3}, \sfrac{1}{3}, \sfrac{1}{3}, 0, \dots, 0]$,
where $T$ includes digits (tokens) 0 to 9 and $\mathcal{U}(2, 5)$ covers all digits (with 0 for unsupported digits). 

\paragraph{Additional Metrics.} We introduce three metrics to understand if there are patterns in the mode.

\textbf{Mode Probability} is the mean max probability of $\Pi$ over the dataset, $\textrm{AVG}_{\textrm{dataset}} \max \Pi$.

\textbf{Mode Stability} is the rate at which the most likely token is preserved between base and chat versions of a model averaged over the dataset,
$\textrm{AVG}_{\textrm{dataset}}(\mathds{1}(\arg\max \Pi_{\textrm{base}} = \arg\max \Pi_{\textrm{chat}}))$.

\textbf{Mode Frequency} examines whether there are biases for particular tokens (numbers). This metric measures the frequency of the mode averaged across distributions. Because different distributions cover different digits, we group the distributions by underlying problem range and inclusivity: E.g., [2, 5) and [132, 135) are grouped. This is equivalent to: (1) setting the temperature to 0 (greedy sampling), (2) averaging over the groups, keeping the digits dimension, (3) taking the maximum for each group, and (4) averaging across all maximums,
$\textrm{AVG}(\max_\textrm{digits}\textrm{AVG}_{\textrm{distributions}, \textrm{ keepdim}}(\Pi^{\tau = 0}))$.

\subsection{Experiment: \texttt{Probabilities}}\label{sec:exp:exp2}
This experiment tests whether the models' output probabilities reflect values in their context.\footnote{\texttt{Probabilities} tests the basic rules of probabilities. As models improve, tests that capture a wider range of probabilities rules would be exciting: Bayes' theorem, De Morgan's Laws, Event Independence, etc.} The following is a representative example of the dataset:

\begin{exe}
 \ex \label{experiments:ex2:1} {From \textbf{17} \textit{red} marbles and \textbf{99} \textit{blue} marbles, Billy reached blindly into the bag and grabbed a marble with the color $[\textit{red}/\textit{blue}]$} 
\end{exe}
 We use 5 templates, 3 numeric scales with 100 configurations each, and 110 pairs of options (e.g., \textcolor{red}{red}/\textcolor{blue}{blue}, or \textcolor{orange}{orange}/\textcolor{C_FIRST}{purple}). The numeric scales are (1) all numbers under 10, (2) ten numbers sampled under 100, and (3) ten numbers sampled under 1000. We these settings bias model behavior. Some factors, such as the numeric context, should influence the model's behavior, while others, such as the ordering of the options, should not.

To simplify the analysis of this large number of configurations, we categorize the model behavior into one of six potential reference points based on WD. In practice, we find that models typically follow one of these six behaviors, making this a useful summary of performance.

\paragraph{Baselines and Reference Points}
We use \texttt{Random} baselines to contextualize our results. For every row in the dataset, the random baseline $\textrm{Random}_{\tau}$ produces a $\Pi$ by uniformly sampling two random numbers from 0 to 1 which are then transformed into a distribution parameterized by a temperature $\tau$ using the softmax function. Second, we observe several behaviors in the results; we create a baseline for each of these behaviors (listed below). \begin{enumerate}[itemsep=0em]
 \item [0.] \texttt{Null:} The PM is too low. This can happen for smaller models like \texttt{Mistral-7B-v0.1}.
 \item [1.] \texttt{Calibrated:} Sets $\Pi = P$, the best case.
 \item [2, 3.] \texttt{Pick Higher:} Sets all probability mass on the $\arg\max \Pi$. This baseline is calibrated directionally: The option with higher probability is correctly preferred but not proportionally. It could alternatively be viewed as mode collapse. Instead of placing all probability mass on the $\arg\max \Pi$, $\texttt{Pick Higher}_{p = q}$ places $q$ (say, 0.7) on $\arg\max$ and $1 - q$ on  $\arg\min$  (0.3). In Appendix \Cref{tab:baselines:prob}, we show performance across a wide range of $p$. (\texttt{Pick Lower} analogously places all probability mass on the $\arg\min \Pi$ (this rarely occurs).
 \item [4, 5.] \texttt{Pick First:} Sets all probability mass on the first option, ignoring numeric information. \texttt{Pick Second:} analogously places all probability mass on the second option.
\end{enumerate}

\section{Results}
\subsection{\texttt{Distributions}}\label{sec:results:exp1}
There are a few patterns across all models. \Cref{tab:exp1} (left) reports the primary metrics. Chat (instruction-tuned) models are less calibrated and have a lower RE than their base counterparts. The base models are more calibrated than the $\textrm{Random}$ baselines. All tested \texttt{gpt-*} models have similar calibration scores to the open-source chat models.

\input{tables/distributions_left}
\input{tables/distributions_right}

The reduced performance of chat models results from their tendency to over-allocate probability on a subset of valid tokens. Result in \Cref{tab:exp1} (right) point to mode collapse. For chat models, the most likely token receives, on average, $66\%$ of the probability mass (up from $28\%$ for base models, beyond the empirical ideal, $23\%$, on this dataset). The most likely token remains the same for $48\%$ instances across base and chat models.

\begin{figure}[ht!]
 \centering
 \input{figures-pgf/over-rep}
 \caption{\textbf{Models Over-represent Some Numbers.} Each bar is the mode frequency, how often the top-chosen token is chosen averaged over distributions. The \textcolor{goldenrod}{gold} lines mark the expected rate for a calibrated model.}
 \label{fig:top-tokens}
\end{figure}



\Cref{fig:top-tokens} reports the mode frequency for two models; Appendix \Cref{fig:top-tokens-full,fig:top-tokens-base,fig:top-tokens-chat,fig:probabilities-base,fig:probabilities-chat} has detailed results. If all probability mass is on valid tokens, the minimum mode frequency is the same as uniform probability; we see much higher rates, ranging from $+29$ to $+50\%$ over the uniform rate. The implication here is that models are also uncalibrated at an outcome level with systematic biases for certain numbers. To give an example, Appendix \Cref{fig:top-tokens-chat} shows that for \texttt{gemma-2-27b}, 3 is the mode for the distribution [0, 7) in $92\%$ of instances. %\footnote{By looking at Appendix \Cref{fig:probabilities-chat}, for \texttt{gemma-2-27b} (chat), we can see that the average probability on 3 for [0, 7) is 0.75, far beyond expectation.}

\begin{dmbox}{\texttt{Distributions}: Systematic Behaviors}
{(1)} Chat models place a majority of probability mass on a subset of valid tokens; \\{(2)} The mode is often stable between base to chat models at the instance level.\\(3) We see poor calibration at the instance level and disproportionate outcomes.
\end{dmbox}


\subsection{\texttt{Probabilities}}\label{sec:results:exp2}
\textbf{High-level results.} All models under-perform simple baselines. $\textrm{Random}_{\tau = 1.0}$ performs better than all models. $\textrm{Pick higher}_{p = 0.7}$, which allocates 0.7 probability mass to the option associated with the higher value, further outperforms all models. Still, the differences between models proves interesting.

There are two key parallels between the results in this section and those in the last section: \textbf{(1)} Instruction tuning decreases the model entropy. The decrease in entropy is often seen via a large increase of probability on the token with the corresponding higher value (replicating \texttt{Pick Higher}). Unlike the previous experiment, this tends to improve the calibration metrics. \Cref{tab:results:probabilities} displays high-level results. \textbf{(2)} Model behavior is systematic (and uncalibrated).  Understanding (2) requires disaggregating the results and examining model behavior across different colors and color orderings.

\input{tables/probabilities}
\begin{figure}[ht!]
 \centering
 % \includegraphics[width=\linewidth]{figures-keynote/the-hard-fig-annotated.pdf}
 \includegraphics[width=\linewidth]{figures-keynote/the-hard-fig-annotated-arr.pdf}
 \caption{
 \textbf{Systematic Patterns in Model Behavior.} The top-left cell of the left heatmap corresponds to instances where \textcolor{orange}{orange} is listed first and \textcolor{gray}{white} is listed second. The heatmap intensity reports which behavior the output probabilities across 100 instances most align with as indicated by the legend. For example, 0.99 in the first cell means that 99\% of the probability mass is on the first option across those 100 instances. \Cref{fig:model_behavior_bar_plot} shows a representative example the top-left cell.
 }
 \label{fig:hard-fig}
\end{figure}

\begin{figure}[ht!]
 \centering
 \includegraphics[width=\linewidth]{figures-keynote/the-examples-figure-arr.pdf}
 \caption{\textbf{Representative Examples of Model Behaviors.} 
 This instance is drawn from \texttt{gpt-4o-mini} results in \Cref{fig:hard-fig}, 
% These instances are drawn from cells in \Cref{fig:hard-fig}.
 %Left, this is an example of \texttt{Pick Second} from \textcolor{goldenrod}{gold} x \textcolor{C_SECOND}{green} cell for \texttt{Llama-3.1-8B}. Right, t
\texttt{Pick First} behavior from the top-left cell.}
 \label{fig:examples-fig}
\end{figure}
\textbf{Further Analysis.}  To make headway, we characterize the high-level behaviors of 
% two models (\texttt{Llama-3.1-8B} and 
\texttt{gpt-4o-mini} in one setting in \Cref{fig:hard-fig} (others in \Cref{app:results:probabilities}). The heatmap in \Cref{fig:hard-fig} is representative for \texttt{gpt-4o-mini}, but its behaviors differs across templates and numeric scales (10s, 100s, etc.), \Cref{app:results:probabilities}
% For \texttt{Llama-3.1-8B} in \Cref{fig:hard-fig}, the model overly favors the second listed color. More broadly, \texttt{Llama-3.1-8B} favors \textcolor{blue}{blue} when it is listed second, and avoids \textcolor{gray}{white}/\textcolor{black}{black}/\textcolor{goldenrod}{gold}. The asymmetry across the diagonal for \texttt{gpt-4o-mini} in \Cref{fig:hard-fig} shows that model behavior can be dependent on word ordering and that there is a hierarchy among the colors.
The diagonal asymmetry means there is a hierarchical, systematic bias for different colors.

We can read the hierarchy from left to right: (Approximately) colors to the left of a color (as ordered in the heatmap) are always preferred by the model \textit{when listed first in the prompt}. However, if the ordering in the prompt is flipped, the model picks the color with associated higher number. So, there are systematic biases conditional on more than one factor. In this particular example, \textcolor{orange}{orange}/\textcolor{magenta}{pink}/\textcolor{C_FIRST}{purple} ``dominate'' most other colors and \textcolor{gray}{white}/\textcolor{brown}{brown} are ``dominated'' by other colors. That the preferences are 1) systematic and 2) hierarchically so was neither required nor expected outcome.

\begin{figure*}[ht!]
 \centering
 \input{figures-pgf/systematic}
 \caption{\textbf{Systematic Patterns in Model Behavior.} Each bar shows the rates of the different behaviors models exhibit averaged across templates, color pairs, and numeric scales.
}
 \label{fig:model_behavior_bar_plot}
\end{figure*}

\Cref{fig:model_behavior_bar_plot} shows behavior rates for each model: \texttt{gpt-*} models (and \texttt{gemma-2-27b}) tend to \texttt{Pick Higher}, others also \texttt{Pick First} and \texttt{Second}. Smaller models exhibit \texttt{null}.

\begin{dmbox}{\texttt{Probabilities}: Systematic Behaviors}
(1) Models often form color hierarchies where the model behavior depends on the word ordering (first or second) and the relative rankings of the words in the hierarchy.\\(2) Model behavior closely aligns with heuristic references, often either \texttt{Pick First} or \texttt{Higher}. In many cases, the heuristic depends on the color ordering.
\end{dmbox}


\section{Human Study}\label{sec:human}
Our experiments above demonstrated that language models are poorly calibrated. Here, we provide further context by comparing the proprietary model and human behavior, asking if models are as random (or not) as people. Previous work suggests that both would be \textit{not} random \citep{}. To get at this question, we use a variation of the two-player game Matching Pennies. We focus on a variation of the game similar to \citet{eliaz2011edgar}. Each round, the ``guesser'' aims to match her chosen coin face with ``misleader's'' choice, earning a +1 reward if their coin faces match, and -1 otherwise. The Nash Equilibrium is for both agents to act randomly. A calibrated model can trivially achieve random behavior.

% Results are presented in Table \ref{tab:exp4_arena}. The two main takeaways are: 1) Models also produce non-random sequences in this setup, further demonstrating their lack of calibration; 2) When prompted, the model's performance improves, and is similar to human performance.

\subsection{Experimental Design}\label{sec:exp:exp4}
This experiment is based on a simple heads/tails game. Our motivation for including this experiment is to allow a human baseline in a setting where random behavior is optimal. This section makes no distinction between calibrated probabilities and unbiased outputs because we don't have access to this information for humans. However, to ``perform'' well, or appear calibrated, requires either the model/person to (1) produce calibrated probabilities which when sampled from will yield random outputs, (2) use an internal random process to produce uncalibrated probabilities that yield random outputs, or (3) have a systematic process for producing outputs that \textit{appear} random enough. (Previous work would suggest that humans are limited in this regard and will likely not be random (and therefore not calibrated).) This leaves us with a one-sided problem. If the humans/models were proficient at producing random outcomes we would have to adjudicate between the above possibilities. 

In a single-round game, the Nash Equilibrium is to select a coin face randomly. We set there to be 100 rounds of play. To focus on calibration, we frame the tested model as the ``misleader.'' The misleader is prompted to submit answers, and the  ``guesser'' is set to predict the misleader's answers. The misleader submits $m_1, m_2, \dots, m_{100}$ answers, and the guesser bases each of its $g_i$ answers incrementeally based upon previous misleader's answers, $\{m_j\,|\, 0 < j < i\}$. We use a n-gram\footnote{Motivated by the strategy here: \url{https://www.expunctis.com/2019/03/07/Not-so-random.html}.} based strategy as our guesser.

\paragraph{Models} We focus on \texttt{gpt-*} models sampling temperature $\tau = 1$. Human behavior is drawn from a sample of 44 games of 100 rounds from $10$ different volunteers with technical backgrounds  up to $10$ different games each.

\paragraph{Additional Metrics} Whereas previous metrics rely on model probabilities, this experiment assumes access only to outputs, meaning  we cannot use the metrics used in previous sections.

\textbf{Player Win Rate (PWR)} is the rate the misleader wins, averaging over 100 games each for up to 100 rounds. The higher this rate, the more random the outputs of the misleader, and thus the more calibrated it is at an outcome level. 

\textbf{Randomness Testing (WW)}. Wald–Wolfowitz \citep{wald1940} tests if the elements of a sequence are mutually independent. Using this test at a significance level of 0.05, we report the proportion of samples that cannot statistically be rejected as non-random, labeling this value as \textbf{WW}. For reference, as shown in Table \ref{tab:exp4_arena} when we sampled random sequences using \texttt{python}, $98\%$ of the sequences could not be rejected; only $7\%$ of human-generated samples could not be rejected. % \footnote{Results with Bartel's test perfectly correlate with the runs test so we only report the runs test.} 

\subsection{Results}
\input{tables/human}

Both best-performing proprietary models and human behavior are not random. Models are prompted with the game rules and we explcility instruct the models (and humans) to be random. Not doing so reduces model performance to near 0. PWR for models and humans are similar, WW for models is higher, but still low.

\Cref{tab:exp4_arena} reports the proportion of samples (where each sample is 100 coin flips) the result could not be considered non-random ($p = 0.05$): Higher WW values suggest the model is more random. More model- than human-generated samples were considered random: $19-43\%$ vs. $7\%$.

\section{Discussion}\label{sec:discussion}
\paragraph{Why Aren't LLMs Already Calibrated?}\label{subsec:whynot}
Should the negative log-likelihood loss endow a pre-trained language model with calibration? If there were $n  \rightarrow  \infty$ examples of Heads and Tails being flipped in the data and the true distribution was reflective of some $p_{\text{heads}}$, then the lowest loss would be achieved via a perfectly calibrated model. Thus, the answer is empirical: What does the training data look like? Finding the disparate scenarios that call for random outcomes may be difficult. Non-calibrated outputs frequently occurring in such scenarios might harm numeric calibration. For example, patterns derived from people preferring the number 7 (out of 10) or 42 (out of 100) or Heads (over Tails) or answering with round numbers ending in 0 or 5 might reduce calibration. Possibly, some models are already capable of producing calibrated results; the models may ``know'' the calibrated output but instead match non-random tendencies, akin to pragmatics. 

\paragraph{Should Models Be Calibrated?} Our work highlights how models that perform well in other types of evaluations fall short in scenarios that call for calibrated outputs. Some may have expected this result given that these models are trained on data generated by people who are also biased. Others might have expected that with the range of data seen in training (data in the wild, code outputs, etc.) models would learn to calibrate. The results are model dependent; for some, there are preferred colors, others overly pick the higher number, and together constitute brittle behavior.

\paragraph{Can We Calibrate Models with Finetuning or Tools?}\label{subsec:ft} We expect that fine-tuning models can improve calibration. Already we show that generic alignment can help, though often with a tradeoff of a large reduction in model entropy. Mitigating mode collapse is a compelling area for future work. Using tools \citep{schick2024toolformer} %, possibly leveraging conformal prediction \citep{shafer2008tutorial}, 
is another practical solution for simple scenarios like those we present, but may not generalize to more complex scenarios.

\section{Conclusion}\label{sec:conclusion}
All models we test are not only \textit{not} calibrated, but behave in different systematically uncalibrated ways. A common theme is that top-performing models (e.g., \texttt{gemma-2-27b} and \texttt{gpt-*} models) \texttt{Pick Higher}, allocating most of the probability mass upon single output token. This is an example of mode collapse. Though mode collapse is commonly studied in computer vision and image generation \citep{thanh2020catastrophic,srivastava2017veegan} \textit{inter alia}, \citet{oattributing} show how RLHF reduces diversity in model outputs, leading to this problem in text generation. Our results are similar: Instruction-tuned models produce valid outputs, but the probability distribution is collapsed to a small portion of the valid answers that are equally correct. While we focus on controlled problem settings, these  issues leave vulnerabilities. For instance, an adversary could leverage that a model is going to behave in a systematically arbitrary manner.

==> archive/distributions.tex <==
\begin{table*}[ht!]
\small
\centering
\begin{tabular}{llrrrrr|rrr}
\toprule
{} & \multicolumn{2}{c}{$\textrm{PM}_\uparrow$} & \multicolumn{2}{c}{$\textrm{RE}_\updownarrow$} &  \multicolumn{2}{c|}{$\textrm{WD}_\downarrow$} & \multicolumn{2}{c}{Mode Prob.} &  \multicolumn{1}{c}{Mode} \\
&            Base & Chat  &  Base & Chat  &         Base & Chat &  Base & Chat & \multicolumn{1}{c}{Stable}  \\
\midrule
Idealized & \multicolumn{2}{c}{1.00} & \multicolumn{2}{c}{1.00} & \multicolumn{2}{c|}{0.00} & 0.23 & 0.23 & -\\
% $\textrm{Random}_{\tau = 0.01}$     &     \multicolumn{2}{c}{0.10} &    \multicolumn{2}{c}{1.00} &  \multicolumn{2}{c|}{0.86} & - & - & - \\
$\textrm{Random}_{\tau = 0.1}$      &  \multicolumn{2}{c}{1.00} &    \multicolumn{2}{c}{0.30} &     \multicolumn{2}{c|}{0.78}& - & - & - \\
$\textrm{Random}_{\tau = 1.0}$      &    \multicolumn{2}{c}{1.00} &   \multicolumn{2}{c}{1.60} &   \multicolumn{2}{c|}{0.38} & - & - & - \\
\midrule
% Meta-Llama-3.1-8B &             1.18 &  0.72 &    0.79 &  0.79 &          0.18 &  0.42 &   0.25 &          0.60 &            0.48 \\
% Mistral-7B-v0.1   &             1.13 &  1.04 &     0.9 &  0.94 &          0.14 &  0.22 &          0.26 &          0.33 &            0.58 \\
% Mistral-7B-v0.3   &             1.13 &  0.50 &    0.89 &  1.00 &          0.14 &  0.57  &          0.26 &          0.65 &            0.35\\
% Mixtral-8x7B-v0.1 &             1.05 &  0.27 &    0.95 &  0.99 &          0.16 &  0.72 &          0.32 &          0.82 &            0.52\\
% Yi-1.5-9B         &             1.11 &  0.49 &    0.87 &  0.95 &           0.20 &  0.61 &          0.30 &          0.75 &            0.40 \\
% Yi-1.5-34B        &             1.06 &  0.39 &    0.93 &  0.90 &          0.21 &  0.62 &          0.37 &          0.75 &            0.53\\
% gemma-2-9b        &             1.17 &  0.48 &    0.85 &  1.00 &          0.15 &  0.59  &          0.22 &          0.66 &            0.40 \\
% gemma-2-27b       &             1.06 &  0.47 &    0.95 &  1.00 &          0.13 &  0.59 &          0.29 &          0.68 &            0.46 \\
Meta-Llama-3.1-8B &    0.81 &  0.79 &             1.16 &  0.68 &          0.17 &  0.44  &          0.25 &          0.60 &            0.48\\
Mistral-7B-v0.1   &    0.91 &  0.94 &             1.12 &  1.04 &          \textbf{0.13} &  0.21 &          0.26 &          0.33 &            0.58 \\
Mistral-7B-v0.3   &     0.90 &  \textbf{1.00} &             1.12 &  0.52 &          \textbf{0.14} &  0.56 &          0.26 &          0.65 &            0.35\\
Mixtral-8x7B-v0.1 &    0.96 &  \textbf{1.00} &             \textbf{1.02} &  0.26 &          0.16 &  0.72  &          0.32 &          0.82 &            0.52\\
Yi-1.5-34B        &    0.95 &  0.92 &             \textbf{1.03} &  0.40 &          0.22 &  0.62 &          0.37 &          0.75 &            0.53 \\
Yi-1.5-9B         &     0.90 &  0.95 &             1.09 &  0.47 &          0.18 &  0.63 &          0.30 &          0.75 &            0.49\\
gemma-2-27b       &    0.96 &  \textbf{1.00} &             1.05 &  0.48 &          \textbf{0.13} &  0.59 &          0.29 &          0.68 &            0.46 \\
gemma-2-9b        &    0.87 &  \textbf{1.00} &             1.16 &  0.47 &          \textbf{0.14} &  0.60 &          0.22 &          0.66 &            0.40 \\
\midrule
$\textrm{AVG}_{\textrm{OpenSource}}$ & 0.91 & 0.96  & 1.09 & 0.57 & 0.16 & 0.58 &  0.28 & 0.66 & 0.48\\
\midrule
gpt-3.5           &     \multicolumn{2}{r}{\textbf{0.99}} &              \multicolumn{2}{r}{\textbf{0.70}} &           \multicolumn{2}{r|}{\textbf{0.42}} & - & 0.53 & -\\
gpt-4-turbo       &     \multicolumn{2}{r}{\textbf{1.00}} &              \multicolumn{2}{r}{0.32} &           \multicolumn{2}{r|}{0.69} & - & 0.79 & - \\
gpt-4o            &     \multicolumn{2}{r}{0.95} &              \multicolumn{2}{r}{0.59} &           \multicolumn{2}{r|}{0.49} & - & 0.58 & - \\
gpt-4o-mini       &     \multicolumn{2}{r}{0.73} &              \multicolumn{2}{r}{0.42} &           \multicolumn{2}{r|}{0.58} & - & 0.73 & - \\

% gpt-3.5           &     \multicolumn{2}{c}{\textbf{0.99}} &              \multicolumn{2}{c}{\textbf{0.70}} &           \multicolumn{2}{c|}{\textbf{0.42}} & - & 0.53 & -\\
% gpt-4-turbo       &     \multicolumn{2}{c}{\textbf{1.00}} &              \multicolumn{2}{c}{0.32} &           \multicolumn{2}{c|}{0.69} & - & 0.79 & - \\
% gpt-4o            &     \multicolumn{2}{c}{0.95} &              \multicolumn{2}{c}{0.59} &           \multicolumn{2}{c|}{0.49} & - & 0.58 & - \\
% gpt-4o-mini       &     \multicolumn{2}{c}{0.73} &              \multicolumn{2}{c}{0.42} &           \multicolumn{2}{c|}{0.58} & - & 0.73 & - \\

% gpt-3.5     &       - &  0.99 &       - &  0.70 &        - &  0.43 & - & 0.53 & - \\
% gpt-4-turbo       &                - &  0.31 &       - &  1.00 &             - &  0.69 & - & 0.80 & - \\
% gpt-4o-mini       &                - &  0.44 &       - &  0.72 &             - &  0.57& - & 0.73 & - \\
% gpt-4o            &                - &  0.60 &       - &  0.95 &             - &  0.49 & - & 0.58 & - \\
\midrule
$\textrm{AVG}_{\textrm{Proprietary}}$  &   \multicolumn{2}{r}{0.92} &  \multicolumn{2}{r}{0.51} &   \multicolumn{2}{r|}{0.54} & - & 0.66 & - \\
\bottomrule
\end{tabular}
\caption{\textbf{\texttt{Distributions} Results.} Metrics described in \Cref{sec:design:metrics,sec:exp:exp1}. \textbf{Left:
(1)} Probability Mass (PM) scores are high for base and chat models, but calibration scores (WD) are lower (better) for base models than chat models. \textbf{(2)} The relative entropy decreased significantly with instruction-tuning to $\sim0.5$ of the ideal value, with \textbf{(3)} the entropy of \texttt{gpt-*} models being similarily low.  \textbf{Right: (1)} Averaged, the probability mass on the top-token for chat models is $+43\%$ above the calibrated ideal, showing where relative entropy increased. \textbf{(2)} The top-tokens remain the same across base and chat models for 48\% of instances. These results together suggest mode-collapse.}
\label{tab:exp1}
\end{table*}

==> archive/distributions_left.tex <==
\begin{table}[ht!]
\small
\centering
% \begin{tabular}{llrrrrr}
\begin{tabular}{@{}l@{}r@{\hspace{4pt}}rr@{\hspace{4pt}}rr@{\hspace{4pt}}r@{}}

\toprule
{} & \multicolumn{2}{c}{$\textrm{PM}_\uparrow$} & \multicolumn{2}{c}{$\textrm{RE}_\updownarrow$} &  \multicolumn{2}{c}{$\textrm{WD}_\downarrow$}  \\
&      Base & Chat  &  Base & Chat  &   Base & Chat  \\
\midrule
Idealized & \multicolumn{2}{c}{1.00} & \multicolumn{2}{c}{1.00} & \multicolumn{2}{c}{0.00} \\
% $\textrm{Random}_{\tau = 0.01}$     &     \multicolumn{2}{c}{0.10} &    \multicolumn{2}{c}{1.00} &  \multicolumn{2}{c|}{0.86} & - & - & - \\
$\textrm{Random}_{\tau = 0.1}$      &  \multicolumn{2}{c}{1.00} &    \multicolumn{2}{c}{0.30} &     \multicolumn{2}{c}{0.78} \\
$\textrm{Random}_{\tau = 1.0}$      &    \multicolumn{2}{c}{1.00} &   \multicolumn{2}{c}{1.60} &   \multicolumn{2}{c}{0.38}  \\
\midrule
% Meta-Llama-3.1-8B & 1.18 &  0.72 &    0.79 &  0.79 &    0.18 &  0.42 &   0.25 &    0.60 &      0.48 \\
% Mistral-7B-v0.1   & 1.13 &  1.04 &     0.9 &  0.94 &    0.14 &  0.22 &    0.26 &    0.33 &      0.58 \\
% Mistral-7B-v0.3   & 1.13 &  0.50 &    0.89 &  1.00 &    0.14 &  0.57  &    0.26 &    0.65 &      0.35\\
% Mixtral-8x7B-v0.1 & 1.05 &  0.27 &    0.95 &  0.99 &    0.16 &  0.72 &    0.32 &    0.82 &      0.52\\
% Yi-1.5-9B   & 1.11 &  0.49 &    0.87 &  0.95 &     0.20 &  0.61 &    0.30 &    0.75 &      0.40 \\
% Yi-1.5-34B  & 1.06 &  0.39 &    0.93 &  0.90 &    0.21 &  0.62 &    0.37 &    0.75 &      0.53\\
% gemma-2-9b  & 1.17 &  0.48 &    0.85 &  1.00 &    0.15 &  0.59  &    0.22 &    0.66 &      0.40 \\
% gemma-2-27b & 1.06 &  0.47 &    0.95 &  1.00 &    0.13 &  0.59 &    0.29 &    0.68 &      0.46 \\
Meta-Llama-3.1-8B &    0.81 &  0.79 & 1.16 &  0.68 &    0.17 &  0.44   \\
Mistral-7B-v0.1   &    0.91 &  0.94 & 1.12 &  1.04 &    \textbf{0.13} &  0.21 \\
Mistral-7B-v0.3   &     0.90 &  \textbf{1.00} & 1.12 &  0.52 &    \textbf{0.14} &  0.56 \\
Mixtral-8x7B-v0.1 &    0.96 &  \textbf{1.00} & \textbf{1.02} &  0.26 &    0.16 &  0.72  \\
Yi-1.5-34B  &    0.95 &  0.92 & \textbf{1.03} &  0.40 &    0.22 &  0.62  \\
Yi-1.5-9B   &     0.90 &  0.95 & 1.09 &  0.47 &    0.18 &  0.63 \\
gemma-2-27b &    0.96 &  \textbf{1.00} & 1.05 &  0.48 &    \textbf{0.13} &  0.59 \\
gemma-2-9b  &    0.87 &  \textbf{1.00} & 1.16 &  0.47 &    \textbf{0.14} &  0.60  \\
\midrule
$\textrm{AVG}_{\textrm{OpenSource}}$ & 0.91 & 0.96  & 1.09 & 0.57 & 0.16 & 0.58 \\
\midrule
gpt-3.5     &     \multicolumn{2}{r}{\textbf{0.99}} &  \multicolumn{2}{r}{\textbf{0.70}} &     \multicolumn{2}{r}{\textbf{0.42}} \\
gpt-4-turbo &     \multicolumn{2}{r}{\textbf{1.00}} &  \multicolumn{2}{r}{0.32} &     \multicolumn{2}{r}{0.69}\\
gpt-4o      &     \multicolumn{2}{r}{0.95} &  \multicolumn{2}{r}{0.59} &     \multicolumn{2}{r}{0.49}  \\
gpt-4o-mini &     \multicolumn{2}{r}{0.73} &  \multicolumn{2}{r}{0.42} &     \multicolumn{2}{r}{0.58} \\

% gpt-3.5     &     \multicolumn{2}{c}{\textbf{0.99}} &  \multicolumn{2}{c}{\textbf{0.70}} &     \multicolumn{2}{c|}{\textbf{0.42}} & - & 0.53 & -\\
% gpt-4-turbo &     \multicolumn{2}{c}{\textbf{1.00}} &  \multicolumn{2}{c}{0.32} &     \multicolumn{2}{c|}{0.69} & - & 0.79 & - \\
% gpt-4o      &     \multicolumn{2}{c}{0.95} &  \multicolumn{2}{c}{0.59} &     \multicolumn{2}{c|}{0.49} & - & 0.58 & - \\
% gpt-4o-mini &     \multicolumn{2}{c}{0.73} &  \multicolumn{2}{c}{0.42} &     \multicolumn{2}{c|}{0.58} & - & 0.73 & - \\

% gpt-3.5     & - &  0.99 & - &  0.70 &  - &  0.43 & - & 0.53 & - \\
% gpt-4-turbo &    - &  0.31 & - &  1.00 & - &  0.69 & - & 0.80 & - \\
% gpt-4o-mini &    - &  0.44 & - &  0.72 & - &  0.57& - & 0.73 & - \\
% gpt-4o      &    - &  0.60 & - &  0.95 & - &  0.49 & - & 0.58 & - \\
\midrule
$\textrm{AVG}_{\textrm{Proprietary}}$  &   \multicolumn{2}{r}{0.92} &  \multicolumn{2}{r}{0.51} &   \multicolumn{2}{r}{0.54}\\
\bottomrule
\end{tabular}
\caption{\textbf{\texttt{Distributions} Results.} Metrics described in \Cref{sec:design:metrics,sec:exp:exp1}. \textbf{
(1)} Probability Mass (PM) scores are high for base and chat models, but calibration scores (WD) are lower (better) for base models than chat models. \textbf{(2)} The relative entropy decreased significantly with instruction-tuning to about half of the ideal value, with \textbf{(3)} the entropy of \texttt{gpt-*} models being similarily low. }
\label{tab:exp1:mode}
\end{table}

==> archive/probabilities.tex <==
\begin{table}[ht!]
\small
\centering
\begin{tabular}{@{}l@{}r@{\hspace{4pt}}rr@{\hspace{4pt}}rr@{\hspace{4pt}}r@{}}
\toprule
% {} & \multicolumn{2}{c}{Rel. Entropy $\updownarrow$} & \multicolumn{2}{c}{Prob. (PM) $\uparrow$} & \multicolumn{2}{c}{Calibr. (WD) $\downarrow$} \\
{}  & \multicolumn{2}{c}{$\textrm{PM}_\uparrow$} & \multicolumn{2}{c}{$\textrm{RE}_\updownarrow$} & \multicolumn{2}{c}{$\textrm{WD}_\downarrow$}\\
 &   Base &  Chat  &    Base &  Chat   &Base &  Chat   \\
\midrule
Idealized &  \multicolumn{2}{c}{1.00}  & \multicolumn{2}{c}{1.00}  &  \multicolumn{2}{c}{0.00} \\
$\textrm{Random}_{\tau = 0.01}$    &     \multicolumn{2}{c}{1.00} &     \multicolumn{2}{c}{0.06} &  \multicolumn{2}{c}{0.69} \\
$\textrm{Random}_{\tau = 0.1}$     &     \multicolumn{2}{c}{1.00} &     \multicolumn{2}{c}{0.50} &  \multicolumn{2}{c}{0.55} \\
$\texttt{pick higher}_{p = 0.7}$   &     \multicolumn{2}{c}{1.00} &     \multicolumn{2}{c}{1.07} &  \multicolumn{2}{c}{0.15} \\
$\texttt{pick higher}_{p = 1.0}$        &     \multicolumn{2}{c}{1.00} &     \multicolumn{2}{c}{0.00} &  \multicolumn{2}{c}{0.47} \\
\midrule
Llama-3.1-8B &    0.38 &  0.80 &    1.08 &  0.90 & 0.54 &  \textbf{0.41} \\
Mistral-7B-v0.1   &     0.30 &  0.54 &     1.10 &  0.74 & 0.59 &  0.50 \\
Mistral-7B-v0.3   &    0.33 &  0.76 &    1.09 &  0.57 & 0.57 &  0.51 \\
Mixtral-8x7B-v0.1 &    0.36 &  \textbf{0.99} &    1.06 &  0.18 & 0.55 &  0.54 \\
Yi-1.5-9B &     0.30 &  \textbf{0.99} &    1.05 &  0.33 & 0.59 &  0.52 \\
Yi-1.5-34B        &    0.41 &  0.61 &    \textbf{1.01} &  0.45 & 0.53 &  0.56 \\
gemma-2-9b        &    0.39 & \textbf{0.99} &    1.14 &  0.49 & 0.53 &  0.54 \\
gemma-2-27b       &    0.54 &  \textbf{1.00} &    1.06 &  0.22 & 0.46 &  0.43 \\
\midrule
$\textrm{AVG}_{\textrm{OpenSource}}$ & 0.38 &     0.84 &  1.07 &      0.49 &       0.55 &      0.50 \\
\midrule
gpt-3.5  &  \multicolumn{2}{r}{\textbf{1.00}} &  \multicolumn{2}{r}{\textbf{0.58}} &        \multicolumn{2}{r}{\textbf{0.32}} \\
gpt-4-turbo       &  \multicolumn{2}{r}{\textbf{1.00}} &  \multicolumn{2}{r}{0.20} &        \multicolumn{2}{r}{0.45} \\
gpt-4o   &  \multicolumn{2}{r}{\textbf{1.00}} &  \multicolumn{2}{r}{0.25} &        \multicolumn{2}{r}{0.42} \\
gpt-4o-mini       &  \multicolumn{2}{r}{\textbf{1.00}} &  \multicolumn{2}{r}{0.35} &        \multicolumn{2}{r}{0.42} \\
\midrule
$\textrm{AVG}_{\textrm{Proprietary}}$ &   \multicolumn{2}{r}{1.00}& \multicolumn{2}{r}{0.35} &  \multicolumn{2}{r}{0.40} \\

\bottomrule
\end{tabular}
\caption{\textbf{\texttt{Probabilities} Results.} \textbf{Takeaways: (1)} Entropy for base models relative to the entropy of a calibrated response is too high (RE above 1.0), whereas for chat models, the entropy is too low (RE below 1.0). However, \textbf{(2)} the chat models tend to place more of the probability mass (PM) on valid tokens and \textbf{(3)} overall the calibration scores are lower (better).}
\label{tab:results:probabilities}
\end{table}






==> archive/submitted_arr.tex <==
\section{Introduction}
We investigate if language model (LM) outputs are calibrated to the numeric content of their contexts. Consider the context below:
\begin{exe}
 \ex \label{intro:example1} {From \textbf{98} \textcolor{blue}{\textit{blue}}  marbles and \textbf{99} \textcolor{red}{\textit{red}} marbles, Tommy reached blindly into a bag and grabbed a marble the color [\textit{\textcolor{blue}{\textit{blue}}/\textcolor{red}{\textit{red}}}]} 
 \end{exe}

This work tests the normative assumption that model probabilities for the next generated token should be calibrated to the relevant numeric content. For example, in \Cref{fig:big-fig}, the probability that an LM continues with one of the \textit{bracketed tokens} should be proportional to the respective \textbf{bolded} values. If the context defines or implies a probability to hold within the context, then subsequent text generation should condition on that probability.


\begin{figure}[h]
 \centering
 \includegraphics[width=\linewidth]{figures-keynote/the-medium-fig-arr.pdf}
 \caption{\textbf{Models are un-calibrated}. 
In this example, \gpt{4o} over-weights the option with a higher count of items beyond the calibrated probability, predicting \textcolor{red}{\textit{red}} with 99.7\% probability when 50.2\% is appropriate. We find consistent patterns of uncalibrated behavior.
}
 \label{fig:big-fig}
\end{figure}

\begin{dmbox}{What Do We Mean By Calibration?}
LMs' output probabilities are \textit{calibrated} to their contexts if the probabilities of relevant tokens correspond to the numeric content implicitly or explicitly defined in those contexts. If tokens $t_1, t_2, \dots, t_n$ are indicated by context $C$ to have probabilities $P = p_1, p_2, \dots, p_n$, a calibrated LM $m$ outputs corresponding probabilities $\pi_i = m(t_i | C)$: 
 \[ p_i \propto	 \pi_i,\quad i\- \in \- 
 1, 2, \dots, n. \]
We set calibration as the distance between $P$ and $\Pi = \pi_1, \pi_2, \dots, \pi_n$ (\Cref{sec:design:metrics}).
\end{dmbox}

Calibration within numeric contexts is a simple concept, but there is good reason to believe that models may struggle with it. Numbers within large pre-training datasets do not all occur with identical frequencies (e.g., numbers ending in 5 appear more than numbers ending in 7), as shown by \citep{zhou-etal-2023-navigating} for the Pile dataset and our findings with Dolmo \citep{soldaini2024dolma} (\Cref{sec:analysis:freq}). These differences may have downstream effects on LMs' biases across different numbers, making it difficult for language models to exhibit calibrated outputs.

Model calibration is related to and impacted by models' mathematical capabilities. Since language models are notably poor in their mathematical capabilities (compared to traditional Question-Answering tasks), it can be challenging for models to be calibrated properly. Roughly speaking, if a model struggles to answer basic math questions, it likely has poor representation and usage of numbers, which are requirements for being properly calibrated. Although models are quickly improving at mathematical reasoning \citep{lin2024rho,shao2024deepseekmath,mathstral2025,chervonyi2025goldmedalistperformancesolvingolympiad}, our work demonstrates that models are not well calibrated even in simple scenarios that require little reasoning.

Because LMs are increasingly used, calibrating LM outputs is increasingly important. We find motivation in a recent explanation method \citep{chen2023models}, Counterfactual simulatability, that requires explanations to capture the ``reason'' a model arrived at an answer. There should be an analogous expectation for model output probabilities. Not reaching this calibration standard may not impact a user over a single interaction; any given outcome is compatible with a calibrated distribution (assuming some probability mass on all options). 

However, failed calibration may have an impact across multiple users or repeat interactions. For example, an uncalibrated model may always recommend visiting a particular restaurant despite the city having hundreds of equally good options. This model's calibration failure could result from something as idiosyncratic as the restaurant's name. In this scenario, the uncalibrated model negatively impacts many parties (e.g., the other restaurants,  customers, etc). This restaurant example is simply one of the many scenarios where users rely on accurate and helpful recommendations (e.g., for movies, job candidates, vacations, colleges, etc). Having correctly calibrated models is critical for situations involving medical or health services, such as making radiology predictions \citep{shreekumar2025x}.

We find that many LMs are poorly calibrated in numeric contexts. Moreover, they fail in systematic ways. In cases like Example \ref{intro:example1}, some uncalibrated models prefer one particular option based on position (e.g., always the first option). Other uncalibrated models may consistently pick the option with the higher number. Word identity of the options and the vocabulary frequency of the numeric information appear to impact these order biases and, thus, the calibration. Our work demonstrates that LMs are often consistently biased in these simple ways. This suggests that there is a risk in relying on LMs for scenarios that involve probabilistic outcomes.

\begin{dmbox}{Contributions}
\begin{enumerate}[leftmargin=*]
 \item Instruction-tuning helps by increasing the model's cumulative probability for all relevant options. Yet, models generally remain poorly calibrated -- sometimes worse than simple baselines.
 \item Models exhibit mode collapse: instruction-tuning overly reduces the entropy of the output distribution.
 \item Models exhibit systematic biases over word identity and order, often overriding the numeric information in the context.
 \item Frequency effects of the number tokens in the training data impact calibration.
\end{enumerate}
\end{dmbox}

\section{Related Work}
\paragraph{Models struggle to calibrate internal uncertainty with textual outputs.}
A related line of work studies how well models calibrate prediction confidence with prediction accuracy: a calibrated model with $0.80$ confidence on each prediction should classify $80\%$ of examples correctly \citep{guo2017calibration, minderer2021revisiting}. Under this definition, \citet{wei2024measuring} reports GPT models have good calibration, whereas, \citet{phan2025humanity} reports the opposite.
Another line of work investigates how well model outputs align with uncertainty \citep{yona2024can,kumar2024confidence,zhou-etal-2023-navigating,lin2022teaching}, termed linguistic calibration \citep{mielke2022reducing}. \citet{yona2024can} reports that models struggle to exhibit internal uncertainty in text. \citet{kumar2024confidence} measures how well confidence is aligned internally (model probabilities) and externally (via eliciting a model to choose among a Likert scale). In our work, we look at the agreement between the probability of predicted outputs and the contextually defined likelihood of outputs in the text. We find that models are often internally \textit{certain} when they should be \textit{uncertain}; this {mode collapse} arises both via supervised fine-tuning and reward-based fine-tuning \citep{oattributing, janus2024modecollapse}. \citet{zhou-etal-2024-relying} also finds that reward-based fine-tuning biases models towards certainty, generating strengtheners (e.g., ``I am certain\dots'') over weakeners (e.g., ``Maybe\dots'').
Notably, faithful calibration is not always desirable; to simplify our experiments, we set aside phenomena like hyperbole and pragmatic effects \citep{tsvilodub2025non}.

\paragraph{Recent work finds that language models struggle to simulate randomness:} coin flip predictions are biased in favor of heads and the first outcome mentioned in context \citep{van2024random}.
\citet{hopkins2023can}, similar to our work, shows that LMs struggle to induce uniform distributions in the 0 to 1 interval.

\paragraph{Biases in language models.} There are large-scale efforts to remove biases from models \citep{rudinger2018,bai2022training}. \citet{pezeshkpour-hruschka-2024-large} shows that LMs prefer multiple-choice options based on their position. Using methods similar to our's, \citet{kusner2017counterfactual} studies probability differences in the setting of counterfactual fairness. We find evidence of similar biases impacting calibration.


\section{Experimental Design}\label{sec:design}
\subsection{Problem Setup}\label{sec:design:problem_setup}
We introduce three templated datasets. Each problem instance is a context $C$ to be continued by a relevant token among $t_1, t_2, \dots, t_n = T \subset V$, where $V$ is the full vocabulary. Each token $t_i$ is associated with an implied probability $p_i$, forming a distribution over $T$, $P = p_1, p_2, \dots, p_n$. In Example \ref{intro:example1}, $T$ is $\{\textrm{\textit{red}}, \textrm{\textit{blue}}\}$ with $P = \{\textrm{\textit{red}} : \sfrac{98}{197}, \textrm{\textit{blue}} : \sfrac{99}{197}\}$. For a model $m$, we define $\Pi = \pi_1, \pi_2, \dots, \pi_n$ where $\pi_i \approx m(t_i | C)$, with one modification. We sum the probabilities of common tokenizations for a given word, namely, capitalization and spaces: $\pi_i = \sum_{s \in \textrm{Tokenizations}(t_i)} m(s | C)$. For example, for the option \textit{red}, we sum probabilities for ``red'', ``Red'', ``\_red'', and ``\_Red.'' This approach does not account for the problem of there being many ways of grammatically continuing the sentence. However, empirically, instruction-tuned models put almost all probability mass on $T$. This admittedly imperfect approach still allows us to study the problem meaningfully.\footnote{See \Cref{app:details} for details on reproducibility.}

\subsection{Metrics and Evaluation}\label{sec:design:metrics}
We use three metrics to test if models calibrate to numeric contexts and where they go wrong.

\textbf{Probability Mass (PM)}: A model's calibration, the relative probability mass across tokens in \textit{T}, is well-founded only if there is sufficient probability mass upon the tokens in $T$. We measure this directly with PM,
$\textrm{PM}(T) \doteq \sum_{t\,\in\,T} \pi_t.$
If $\textrm{PM}(T)$ for a model is low (say, 0.30), then it is unclear if the model is capturing the intended relationship between the context and $T$. While meaningful distribution across $T$ could still exist if these values were normalized, we set this case aside. When $\textrm{PM}$ is high (say, $>0.75$), we can start to meaningfully ask questions about how probability mass is allocated among, say, \textit{red} and \textit{blue}. 

\textbf{Wasserstein Distance (WD)}: To measure {calibration}, we use {WD} \citep{kantorovich1939mathematical}, which captures the movement between one distribution (or set of values) and another.\footnote{Kullback–Leibler (KL) divergence is also a natural choice. However, some problems in our datasets include options with the value zero where KL would be undefined. We also compute Mean-Squared Error (MSE) but don't find a material difference in the findings so we only report the WD.} 

\textbf{Relative Entropy (RE):} To help understand a model's behavior, we propose $\textrm{RE} = \textrm{H}(\Pi) - \textrm{H}(P)$, the difference in entropy $\textrm{H}$ between model and ideal calibrated probabilities. $\textrm{RE}<0$ means the model's probabilities are overly concentrated and $\textrm{RE}>0$  means they are overly diffuse.

\subsection{Models} Our experiments assume access to model logits.
We test range of open-source models with both base and instruction-tuned versions available: \mistral{1}, \mistral{3}, \mixtral{}, \yi{9}, \yi{34}, \llama{}, \gemma{9}, \gemma{27} \citep{jiang2023mistral,jiang2024mixtral,young2024yi,dubey2024llama,team2024gemma}; and four proprietary models, \gpt{3.5}, \gpt{4-turbo}, \gpt{4o-mini}, and \gpt{4o} \citep{brown2020language,achiam2023gpt,openai2023gpt4o}. We prompt instruction-tuned models to calibrate outputs to the numbers in context. We refer to the base version of the models as ``Base'' and the instruction-tuned, prompted models as ``Chat.''

\subsection{Datasets}
We introduce three datasets \textit{colors}, \textit{wordproblems}, and \textit{distributions}. The following are representative examples, respectively: \footnote{Our datasets test basic ratios and probability. As models improve, it would be exciting if datasets targeted concepts like Bayes' theorem, De Morgan's laws, event independence, etc.}

\begin{exe}
 \ex \label{experiments:ex2:1} {From \textbf{17} \textit{red} marbles and \textbf{99} \textit{blue} marbles, Billy reached blindly into the bag and grabbed a marble with the color $[\textit{red}/\textit{blue}]$}
\ex \label{experiments:ex2:2} There was a grove with \textbf{17} \textit{spruce} and \textbf{99} \textit{cedar}. During a thunderstorm lightning struck a tree. All the trees were about the same height and elevation. Turned out, the species of the tree was [\textit{spruce/cedar}]
\ex \label{experiments:ex2:3} Sampling from a uniform distribution with support from \textbf{2} inclusive to \textbf{5} exclusive, I sampled the number $[\textit{0}/\textit{1}/\textit{\textbf{2}}/\textit{\textbf{3}}\dots\textit{9}]$
\end{exe}

For \textbf{(a)} \textit{colors}, we use 5 templates, 3 numeric scales with 100 configurations each, and 110 permutations of color options (e.g., \textcolor{red}{red}/\textcolor{blue}{blue} and  \textcolor{blue}{blue}/\textcolor{red}{red}).\footnote{Calibration could be well-studied by sampling non-exhaustively across these permutations but doing so lets us highlight biases across different options.
} The numeric scales are (1) numbers 1 to 10, (2) ten numbers sampled from 10 to 100, and (3) ten numbers sampled from 100 to 999. Pilot experiments with larger numbers ($>1000$) did not see marked differences in calibration. Still, future work should study a wider range of numbers. For \textbf{(b)}  \textit{wordproblems}, there are 10 templates, the same 3 numeric scales with 100 configurations each, and 4-10 pairs of options (e.g., \textit{spruce/cedar}, or \textit{nurse/doctor}) depending on the template. For \textbf{(c)} \textit{distributions}, the configuration is different. The task is to pick a number uniformly from an interval. The valid options in \textit{T} are all integers in the interval. There are 5 templates, different range inclusivities, and 320 pairs of numbers that define the intervals ranging from 10 to 1000. Each problem is set to occur within an interval length of less than 10 and requires only a single token prediction.

When we compute standard errors we cluster option pairs together \citep{miller2024adding}. All our results show the 95\% confidence interval (not the standard error) either explicitly or using $\pm$ notation.

\input{tables/arr_dataset}

\subsection{Reference Behaviors and Baselines}
\noindent\textit{Reference Behaviors.} Understanding a model's behavior across many instances is difficult. However, models typically produce one of six behaviors in practice, making them a useful way to summarize model behavior. We categorize the model behavior into these as reference points.

Summaries are limited: For instance, we find that for \gpt{4o-mini} when the color \textit{white} is listed second in the prompt, that first color is always picked. This is classified as Pick First but could be instead understood as ``pick the first color before options starting with \textit{w}.'' Our reference points describe behavior compatible with a model's behavior over many examples and settings, but it is still only descriptive. Finally, for a single instance, there are multiple valid explanations (e.g. in Example \ref{intro:example1} could be Pick Higher or Pick Lower). We can only determine the behavior over a large set of balanced instances.
\begin{enumerate}[itemsep=0em]
 \item [0.] \texttt{Null:} PM is closer to zero than to any reference behavior.
 \item [1.] \texttt{Calibrated:} Sets $\Pi = P$, the best case.
 \item [2.] \texttt{Pick Higher:} Sets all probability mass on $\arg\max P$.
 \item [3.] \texttt{Pick lower:} analogously sets all probability mass on $\arg\min P$.
 \item [4.] \texttt{Pick First:} Sets all probability mass on the first option, ignoring numeric information.
 \item [5.] \texttt{Pick Second:} analogously sets all probability mass on the second option.
\end{enumerate}

\noindent\textit{Baselines.} We introduce two more baselines besides using the reference behaviors above as baselines. First, $\texttt{Pick Higher}_{p = q}$ places $q$ (say, 0.7) on $\arg\max P$ and the remainder of the probability mass evenly across other tokens in $T$. Second, \texttt{Random} baselines to contextualize our results. For every problem in the dataset, the random baseline $\textrm{Random}_{\tau}$ produces a $\Pi$ by uniformly sampling two random numbers from 0 to 1, which are then transformed into a distribution parameterized by a temperature $\tau$ using the softmax function. 


\section{Results}\label{sec:results:exp2}

\subsection{Probability Mass}
First, we closely examine the probability mass (PM) on the relevant tokens. Consider Example \ref{intro:example1} where \gpt{4o} is to pick either \textit{Red} or \textit{Blue}. 
There, a high PM means that the model successfully allocated probability mass over these tokens. Success depends on the design of our problem scenarios and model capability. The high scores suggest that the models correctly interpret the basic task.

\input{tables/arr_pm}

\Cref{tab:results:pm} reports PM for the base and chat versions of all tested models. \textbf{Instruction-tuned models have statistically significantly higher PMs over their base versions.} This can be seen by the strictly positive 95\% confidence intervals of the difference between the chat and base scores in the rightmost column. Except for \llama{} and \yi{34} on \textit{distributions}, this holds for all models. The instruction-tuned PM scores are all reasonably high, suggesting that the datasets' sentence templates are well-formed. The primary exception is \mistral{1}. Notably, gpt-* models had lower PM on \textit{wordproblems}.

\input{tables/arr_wd_3}
\subsection{Calibration}
Next, we examine the calibration scores of instruction-tuned models in \Cref{tab:results:wd}. Given the low PM scores of the base models, we leave those results to Appendix \Cref{tab:results:wd:all}. Our high-level finding is simple: all tested models are poorly calibrated, and their performance is typically worse than simple baselines. Some models are mildly better than a baseline that sets 100\% probability to the option associated with the higher number, but most are not. Another baseline, Pick $\textrm{Higher}_{p = 0.7}$, which allocates 70\% probability to the option associated with the higher number, outperforms all models. This result, more than anything, describes the best average output probabilities for \textit{colors} and \textit{wordproblems}.
This all goes to say: \textbf{Although the models can allocate probability mass on valid options, they cannot properly allocate probability mass \textit{among} these options in a calibrated manner.}
In \Cref{app:results:reproducibility}, we find evidence that our calibration results are stable across a broader range of templates and template variations.




\subsection{Relative Entropy}
\input{tables/arr_re_3}
The section above demonstrated that the models cannot allocate the probability mass \textit{among} the valid options in a calibrated manner. Here, as shown in \Cref{tab:results:re}, we find that these models fail primarily by over-allocating probability mass on one of the two options: mode collapse. Every model's RE was statistically significantly less than the calibrated result, often with large effects for \textit{colors} and \textit{wordproblems}. Models with the best calibration scores (gpt-* models) also have the lowest relative entropy, suggesting no model approaches well-calibrated behavior. 

Instruction-tuning appears to cause this mode collapse. Across all three datasets, there is a drastic reduction in entropy between the base and chat model versions, on average, 0.50/0.36/1.19 bits across the three datasets respectively. This drop in bits reduces the entropy to 47/42/55\% percent of the entropy of the ideal calibrated result. (See \Cref{app:results:mode} for more details.)

\section{Analysis: Option Identity and Order}\label{sec:analysis:option}
\begin{figure}[ht!]
 \centering
 \includegraphics[width=\linewidth]{figures-keynote/the-hard-fig-annotated-arr.pdf}
 \caption{
 \textbf{Systematic Patterns in Model Behavior.} Each cell corresponds to model behavior across 100 examples. The number is the rate the outputs are compatible with the given behavior. For example, 1.00 in the first top-left cell means that for 100/100 instances a majority of the probability mass is on the first option. The top-left cell corresponds to instances where \textcolor{PURPLE}{purple} is first in the prompt and \textcolor{gray}{white} is second. High rates across multiple behaviors are impossible; they are mutually exclusive across the 100 instances. See \Cref{fig:examples-fig} for a representative instance drawn from the top-left cell.
 }
\label{fig:hard-fig}
\end{figure}
In this section, we study the particular behaviors that models exhibit on the \textit{colors} dataset, finding that \textbf{the models exhibit systematic biases and preferences based upon word identity and word order.}
Understanding that (1) the models are poorly calibrated and (2) exhibit low entropy falls directly out of our proposed metrics. However, understanding how the models behave is more complicated. To start, we characterize the behavior of \gpt{4o-mini} in \Cref{fig:hard-fig} (more in \Cref{app:results:ordering}). \Cref{fig:model_behavior_bar_plot} shows model behavior across all settings.

\begin{figure*}[ht!]
 \centering
 \input{figures-pgf/systematic}
 \caption{\textbf{Systematic Patterns in Model Behavior} for the \textit{colors} dataset. Each bar shows the percent of the different behaviors models exhibit averaged across templates, color pairs, and numeric scales.
}
 \label{fig:model_behavior_bar_plot}
\end{figure*}

Beyond the specific systematic patterns we uncover, we want to stress that the existence of these patterns is important. Every use case of LMs that requires such choices may have similar patterns. \textbf{That these systematic errors arise even with innocuous features like color should give us pause about using models to make probabilistic choices in more complicated scenarios.}

\Cref{fig:hard-fig} captures model behavior across all tested pairs of color options. The most apparent note to make is the diagonal asymmetry. \textbf{This asymmetry shows a hierarchical, systematic bias across word identity (specific colors) and word order.} Each cell within the heatmap reports the rate at which the model's output probabilities are compatible with the given behavior across a full grid of number pairs. The behavior with the highest compatibility rate is displayed and indicated by the color. For example, if the model had rates of 100 for Pick first, 50 for Pick higher, and 50 for pick second, the plot would show the rate of 1.00 (100/100) for Pick first. A high rate of two behaviors cannot happen because the 100 examples are balanced (in half, the first number is higher, in the other half, the second number is higher.) 

\begin{figure}[ht!]
 \centering
 \includegraphics[width=\linewidth]{figures-keynote/the-examples-figure-arr.pdf}
 \caption{\textbf{Representative Examples of Model Behaviors.}
 This instance is from \gpt{4o-mini} results in \Cref{fig:hard-fig}, \texttt{Pick First} behavior from the top-left cell.}
 \label{fig:examples-fig}
\end{figure}

The behaviors exhibited across the diagonal are often different.
This means that option order, listing a color first or second, greatly affects calibration. For example, in \Cref{fig:hard-fig}, we can see that when ``white'' is mentioned first, the model tends to Pick Higher and when it is mentioned second, the model tends to Pick First. Because Pick Higher is a more calibrated behavior than Pick First, mentioning ``white'' first leads to lower calibration scores.

We measure these differences in calibration across options and models, detailing our findings in \Cref{app:results:ordering}. There is some shared correlation between color orderings among similar models (\gpt{4o}/\gpt{4o-mini}), suggesting that training data plays a large role in forming these patterns of behavior.

To give a high-level picture, in \Cref{fig:model_behavior_bar_plot}, we report the overall behavior rates for each model. \Cref{app:results:ordering} details how we compute the proportions of different behaviors across the dataset.
\gpt{*} models (and \gemma{27b}) tend to \texttt{Pick Higher}, others also \texttt{Pick First} and \texttt{Second}. Smaller models also exhibit \texttt{null}. These patterns (1) differ across models (whether it is Pick First or Second vs Pick Higher or something else) but (2) the word identity (\textcolor{red}{\textit{red}}/\textcolor{gray}{\textit{white}} with the same numeric information) consistently interacts with word order (\textcolor{red}{\textit{red}}/\textcolor{gray}{\textit{white}} vs \textcolor{gray}{\textit{white}}/\textcolor{red}{\textit{red}}) to create systematic error patterns per model.

\input{tables/arr_freq}

\section{Analysis: Number Token Frequency}\label{sec:analysis:freq}
\paragraph{Numbers appear at different frequencies in training data. Does frequency explain the differences in calibration?}  We find that the models exhibit different behaviors, but there are three primary patterns. Across almost all models, there is a high and significant correlation between number frequencies and average calibration scores.
\begin{exe}
 \ex {From \textbf{50} {\textit{blue}}  marbles and \textbf{84} \textit{red}$\dots$}
\end{exe}
\noindent Repeating a partial example similar to those above, here, in this section, we focus our analysis on the numeric content, here $N_1=50 $/$ N_2=84$, particularly the frequencies of those numbers in the training data. Because the models we test do not publish their training data details, we approximate the frequency of numbers in their training data using infini-gram\footnote{\url{https://infini-gram.io/api_doc.html}} \citep{liu2024infini} over Dolma \citep{soldaini2024dolma}, a 3 trillion token corpus. Given the limited amount of natural text available online, we expect pre-training datasets to overlap significantly and be similarly distributed.\footnote{ We query for the number counts with spaces both before and after each number: ``\_$N$\_'', to account for numbers appearing within other numbers. This assumes the noise we introduce here is distributed similarly across numbers.} 

We use the Spearman's correlation between the calibration scores and the \textit{Frequency Gap}, the log absolute difference of the number frequencies, $\log|(\textrm{Freq}(N_1) - {\textrm{Freq}(N_2)}|$.\footnote{See \Cref{app:results:freq} for more results and correlations.} Using the Frequency Gap is a simple way to capture if there is a relationship between the frequencies of the two numbers.

We present the correlation results in \Cref{tab:freq}.
Frequency effects appear to negatively impact the base models: Larger Frequency Gaps correlate with worse calibration. Conversely, frequency effects appear to positively impact instruction-tuned models: Larger Frequency Gaps correlate with improved calibration. Frequency effects on \textit{distributions} are different. Effects are weaker, and increased frequency tends to improve calibration.

Frequency effects are a known issue for LMs \citep{wei2021frequency,lovering2023training,mccoy2024embers}; \textbf{Our results reinforce the understanding that increases in model scale and performance have not canceled out such biases.}


\section{Conclusion}\label{sec:conclusion}
All models we test are not only \textit{not} calibrated; they are generally less calibrated than simple baselines.
Word identity, word order, and the vocabulary frequency of the numeric information heavily modulate model behavior. Even in the basic problem settings we test in this paper, LMs are biased in simple ways, which suggests significant risks in using models in probabilistic scenarios to make decisions.

\section*{Limitations}
This work strikes a balance between sampling across a large space of options--more numbers \citep{shrestha2025mathematicalreasoninglargelanguage}, more unique templates--and uncovering biases present in those chosen options, which benefits from a ``grid-search'' approach. Future work that increases the diversity and size of these datasets could only improve this line of work.

We report Spearman's correlation in \Cref{sec:analysis:freq}. Using mixed-effects models may provide additional insights. Increasing the range of numbers used, especially in this section, could improve the robustness of our results.

\section*{Potential Risks}
This work does not pose a risk. Instead, this work highlights several risks of using uncalibrated models and shows that current models are uncalibrated even in simple settings.
